S2TD: a Separation Logic Verifier that Supports Reasoning of the Absence and Presence of Bugs

Heap-manipulating programs are known to be challenging to reason about. We present a novel verifier for heap-manipulating programs called S2TD, which encodes programs systematically in the form of Constrained Horn Clauses (CHC) using a novel extension of separation logic (SL) with recursive predicates and dangling predicates. S2TD actively explores cyclic proofs to address the path explosion problem. S2TD differentiates itself from existing CHC-based verifiers by focusing on heap-manipulating programs and employing cyclic proof to efficiently verify or falsify them with counterexamples. Compared with existing SL-based verifiers, S2TD precisely specifies the heaps of de-allocated pointers to avoid false positives in reasoning about the presence of bugs. S2TD has been evaluated using a comprehensive set of benchmark programs from the SV-COMP repository. The results show that S2TD is more effective than state-of-art program verifiers and is more efficient than most of them.

==> ae.tex <==
We describe artifact of our accepted paper at CAV 2016. The steps are as follows.
First, download the virtual machine (VM) with our tools and artifact at:
https://dl.dropboxusercontent.com/u/7749529/s2_ae.ova
Second, run this VM with a VM Manager, e.g. VirtualBox 5.1.20;
Username: loris7, Password: loris7.
In this VM, our folder is located at /home/cav/cav2017-ae/.
This folder contains: our accepted paper (cav2017-53.pdf), a detailed README
file, and artifact folder (act). The README file has four sections.
The first section presents the structure of the cav2017-ae folder.
The next three sections show how to reproduce the experimental results
in Table 1, Table 2 and Table 3, respectively.
The last section describes how to run our tools with a new input.
In the README file, lines starting with ">" are terminal commands;
to run these commands, copy and paste the text (excluding ">") into Terminal and press enter.
After running our VM, open the Terminal, change the current directory to 
/home/cav/cav2016-ae/art/, read README and let start.


==> app.tex <==
%% \section{Artifact Evaluation}\label{app.s2vm}
%% \input{s2vm.tex}

%% \section{Illustrative Example (Cont)} \label{mov-leak}
%% \input{mov-leak}


%% \section{Proof of Lemma 5.2}\label{proof.elim} %% \ref{lem.elim}
%%   \input{proof-ex-elim}

%% \subsection{More Examples}\label{app.more.examples}
%% \input{more-ex}

%% \section{Proof of Lemma \ref{lem.sat.base}}\label{proof.lem.sat.base}
%% \section{Decidable Fragment {\slap}}\label{deci.frag}
%% \input{deci-frag}

%\section{Proof of Lemma \ref{lem.sat.base} }\label{proof.lem.sat.base}

%\section{Proof of Termination }\label{proof.thm.term}
To prove  Lemma \ref{thm.term}, we first prove some auxiliary lemmas.
\input{sat-term-main}




%% \subsection{Proof of Lemma \ref{lem.shape}}\label{proof.lem.shape}
%%  \input{proof-term-shape}

%%  \subsection{Proof of Lemma \ref{thm.term}}\label{proof.thm.term}
%%  \input{proof-term}

%% The correctness of Theorem \ref{thm.term}
%%  immediately follows the following Lemma lemma \ref{lem.arith},
%% lemma \ref{lem.shape}
%% and the results in \cite{Marius:CAV:2010,Makoto:APLAS:2016}
%% which state that the transitive closure of these periodic relations is Presburber-definable
%%  and effectively computable.

%% \subsection{Complexity} \label{proof.compl}
%% \input{complexity}


==> complexity.tex <==
\hide{Let \form{\D_{sh}{\equiv}\exists \setvars{w}{\cdot}\sepnodeF{x_1}{c_1}{\setvars{v}_1}{\sep} ...{\sep}
\sepnodeF{x_n}{c_n}{\setvars{v}_n}{\wedge}\atom}
be a base formula whose pure part is restricted to (dis)equality.
Let \form{\pure_{sh}{\equiv}{\xpure}({\D_{sh}}){\equiv}\exists\setvars{w}{\cdot} \atom_{sh}}.
We use \form{\projectpe{\atom_{sh}}{\setvars{w}}}
to denote an exhaustive quantifier elimination, i.e. \form{\atom_0{\equiv}\projectpe{\atom_{sh}}{\setvars{w}}} and
 \form{\FV(\atom_0){\cap} \setvars{w}{=}\emptyset}.
Given an inductive predicate \form{\code{U_i}(\setvars{v}_i)}, let \form{m_i} be
 its arity plus one,
  \form{\exists \setvars{w} {\cdot}\D} be derived from unfolding tree of 
\form{\code{U_i}(\setvars{v})}, and
\form{\atom_{0}{\equiv}\projectpe{\xpure({\D})}{\setvars{w}}}. We have
 \form{\FV(\atom_{0})~ {\subseteq}~ \setvars{v}_i {\cup} \{\nil\}}.
As \form{\atom_{0}} is restricted in (dis)equality,
the maximum number of conjuncts 
of \form{\atom_{0}} is \form{{2m^2_i}}.
%
Given a set of assumptions \form{\Horn} based on
a  system of \form{N} inductive predicates. Suppose
the possibly longest (number of conjuncts) relational constraint:
\saveone\[\saveone
\form{\exists \setvars{w}_k{\cdot}\sepnodeF{x_1}{c_1}{\setvars{v}_1}{\sep} ...{\sep}
\sepnodeF{x_n}{c_n}{\setvars{v}_n}{\sep}
{\code{U_1}(\setvars{v}_1){\sep}..{\sep}{\code{U_N}(\setvars{v}_N)}}
{\wedge}\atom ~{\imply}~ \code{U_k}(\setvars{v}_k)}
\]
Thus, the computational complexity for {\sat} ({\unsat}) is 
$\mathcal{O}(N2^{2m^2})$ (resp., $\mathcal{O}(2^{2m^2})$) where
 \form{m} is maximum arity plus one.}

\begin{proof}
Two sequence \form{\setvars{v}} and \form{\setvars{t}}
have the same sequence of observable variables
if for all valid position \form{k} then \form{\setvars{v_k}}
is an observable variable or \form{\nil} and \form{\setvars{t_k}{=}\setvars{v_k}}.

Suppose \form{\indsh_i} and \form{\indsh_j}
be two inductive formulas in the unfolding tree derived for \form{\indsh_0}.
Let \form{\indsh_i{\equiv}\exists \setvars{w}_i{\cdot}\base_i{\sep}
{\code{P_1}(\setvars{v}_{i_1}){\sep}..{\sep}{\code{P_{N}}(\setvars{v}_{N_i})}}}
and \form{\indsh_j{\equiv}\exists \setvars{w}_j{\cdot}\base_j{\sep}
{\code{P_1}(\setvars{v}_{j_1}){\sep}..{\sep}{\code{P_{N}}(\setvars{v}_{N_j})}}}.
(We discard the inductive predicate instances whose all actual parameters
are existentially quantified as they will not attribute to the satisfiability.)
Two these node are linked together if they produce the same set of
(dis)equality conjunctions.
This happens if the following conditions hold.
First, \form{\exists \setvars{w}_i{\cdot}\base_i} and
\form{\exists \setvars{w}_j{\cdot}\base_j} are reduced to
an identical (dis)equality conjunction. Second,
for each predicate instance \code{P_k}, for all
\form{k \in 1..N}, \form{\code{P_k}(\setvars{v}_{i_k})}
and
\form{\code{P_k}(\setvars{v}_{j_k})} have the same sequence of observable
variables.
The complexity for the first condition is  $\mathcal{O}((2^{2m^2}))$.
The complexity for the second condition for each inductive predicate
instance is  $\mathcal{O}((2^{m})$
and for \form{N}  inductive predicate
instances is  $\mathcal{O}((2^{m})^{N})$.
\qed
\end{proof}


==> correct.tex <==
As shown in \cite{Loc:2014:S2SAT:TR},
{\algonamesl} always terminates for {\sat}.
In this subsection,
we prove that {\algonamesl} terminates for an {\unsat}
shape-based formula. %% Our termination proof is based on the fact that
%% an inductive shape-based formula \form{\indsh} can not be unfolded forever.
We prove that
for each leaf of the unfolding tree derived for an {\unsat} formula
if it is not {\unsat}, it must be linked back to form a cyclic proof
in {\em finite} steps.
%%  While we describe the proof
%% for the inputs containing one inductive predicate
%% instance, the proof for the input with multiple inductive predicate
%% instances is straightforward using induction.
Let  \form{\indsh_0} be the input.
%% be as: \form{\indsh_0 {\equiv} \exists \setvars{w}{\cdot}\base{\sep}
%% {\code{P_1}(\setvars{v}_1)}}.
Let \form{\setvars{v}{=}\FV(\indsh_0)}. %%, and \form{\setvars{v}{\cap}\setvars{w}{=}\emptyset}.
We use {\em observable} (resp., {\em unobservable}) 
 variables %%(i.e., \form{\setvars{v}})
to denote free (resp., existentially quantified) variables.
%% and existentially quantified variables %% (i.e., \form{\setvars{w}})
%%  are denoted as {\em unobservable} variables. 
 The core of our proof is
 that satisfiability of base formulas in this fragment
is equiv-satisfiable to a (dis)equility conjunction
over {observable} variables,
but not {unobservable} variables.
Thus, the set of based formulas derived from unfolding tree
of \form{\indsh_0}
relies on observable variables of \form{\indsh_0}.
Recap that an open leaf \form{\indsh_i} is linked back to
an internal node \form{\indsh_i}
if the set of base formulas derived from it is identical to the set from \form{\indsh_i}.
As the number of (dis)equality conjunctions over
 observable variables of the root \form{\indsh_0} is finite,
this back-link must be formed in finite steps.

 Recall that solving a formula
primarily relies on functions \form{\xpure(..)} and \projectp{..}{..}.
%% \form{\satb{{\exists \setvars{w} {\cdot}\D^b}}{~\equiv~}\satp{\projectp{\xpure(\norm{\D^b})}{\setvars{w}}}}.
We show that a base formula in this fragment is equi-satisfiable to
a (dis)equality conjunction over its observable variables.
\begin{lemma}[Equiv-SAT Reduction \cite{Loc:2014:S2SAT:TR}]\label{lem.sat}
Let \form{\D^b} be a base formula,
 \form{\forall \sstack{,}\sheaps \cdot \sstack{,}\sheaps ~{\force}~ \D^b} ~iff~
  \form{\exists \sstack' \cdot \sstack \subseteq \sstack' \text{ and } \sstack'~ {\force}~ {\xpure}({\D^b})}.
\end{lemma}
%
\begin{defn}The projection \projectpsh{\atom_{sh}}{\setvars{w}} to eliminate
the existential quantifiers
\form{\setvars{w}} id defined for equality as follows.
\form{ \projectpsh{\true}{\setvars{w}} = \true}. Otherwise,
\savespace\[\savespace
\begin{array}{l}
 \projectpsh{v_1{=}v_2{\wedge}\atom_1}{\setvars{w}} =
  \begin{cases}
    \atom_1       & \quad \text{if } v_i\in\setvars{w}, i=1,2\\
    \atom_1[v_1/v_2]  & \quad \text{if } v_1\in \setvars{w} \text{ and } v_2 \not\in \setvars{w}\\
    \atom_1[v_2/v_1]  & \quad \text{if } v_2\in \setvars{w} \text{ and } v_1 \not\in \setvars{w}\\
    v_1{=}v_2{\wedge}\atom_1 & \quad \text{otherwise}
  \end{cases}
\\
 \projectpsh{v_1{\not=}v_2{\wedge}\atom_1}{\setvars{w}} =
  \begin{cases}
    v_1{\not=}v_2{\wedge}\atom_1       & \quad \text{if } v_i{\not\in}\setvars{w}, i=1,2\\
    \atom_1 & \quad \text{otherwise}
  \end{cases}
\end{array}
\]
\end{defn}
We assume that \form{\atom} is sorted s.t. equality conjuncts are processed before disequality ones.
\begin{lemma}[Equiv-SAT Elimination]\label{lem.elim}
 \form{\exists\setvars{w} {\cdot}\atom} is satisfiable iff \projectpsh{\atom}{\setvars{w}}  is satisfiable.
\end{lemma}
The proof for this lemma which is based on induction on the size of \form{\atom}
is presented in App. \ref{proof.elim}.
The following theorem immediately follows the discussion above.
\begin{theorem}[Termination]\label{thm.bound}
{\algonamesl} terminates for shape-based formulas.
\end{theorem}


Given an inductive formula \form{\indsh} including \form{m}
observable variables plus one, the number of equality conjunctions over these variables
and \form{\nil}
is \form{2m^2}. It can be implied that the maximum number of
observable parameters of each inductive predicate instances in
is \form{\indsh}.
As so, we show the complexity result in the following theorem.
\begin{theorem}[Complexity]\label{thm.bound}
Suppose
\form{\indsh_0{\equiv}\exists \setvars{w}_k{\cdot}\base{\sep}
{\code{P_1}(\setvars{v}_1){\sep}..{\sep}{\code{P_N}(\setvars{v}_N)}}}
be a shape-based unsatisfiable formula and
 m be the number of its observable variables plus one.
Complexity of {\algonamesl} to solve \form{\indsh_0} is
  $\mathcal{O}((2^{2m^2})\times(2^{m})^{N})$
\end{theorem}
A proof is discussed in App. \ref{proof.compl}.
We remark that the satisfiability problem of shape-based formulas
is not new. Its decidability was presented in \cite{Brotherston:LISC:14}.
Our main contribution is the decision procedure based on {\algonamesl}.


==> cyclic-ex-ll.tex <==

Consider the satisfiability check for the formula 
\form{\D_1 \equiv \seppred{\code{ell}}{x,n} \wedge n{=}5}.

To illustrate, consider the formula:
 \form{\D_0 {\equiv} \seppred{\code{list}}{x_0{,}n_0} {\wedge} n_0{<}0},
 \savespace\[ \savespace
\begin{array}{l}
\seppred{\code{list}}{x{,}n} ~{\equiv}~ \emp {\wedge} x{=}\nil {\wedge} n{=}0) \quad ~|~  x{=}\nil {\wedge} n{=}0\\
 \quad \quad \vee~
(\exists q{,}n_1 {\cdot}~ \sepnode{x}{node}{q{,}n_1} {\sep} \seppred{\code{list}}{q{,}n_1} {\wedge} n_1{=}n{-}1) \quad |~ x{\neq}\nil \\
\quad \invo~ \true;
\end{array}
\]
\noindent Derivation proof for this formula is presented in
Fig. \ref{fig.unfold.cyclic}.
\form{\D_{12} {\equiv} \exists q_1{,}n_1 {\cdot}~ \sepnode{x_0}{code}{q_1{,}n_1} {\sep}
 \seppred{\code{list}}{q_1,n_1}  {\wedge} n_1{=}n_0{-}1}.
(The first branch of \code{list} has been pruned when unfolding \form{\D_0}
 as it does not satisfy the context \form{n_0{<}0}).
After substituted, \form{\D_{12}} could be linked back to \form{\D_0},
  \form{\D_{12}} is marked as close and form
a cyclic proof for \form{\D_0}.
%%\form{\sstate_{i} {=} \{ \}}, \form{\sstate {=} \{ \}}.
Thus, {\algoname} returns {\unsat}.


==> cyclic-ex.tex <==

To illustrate, consider the formula:
 \form{\D_0 {\equiv} \seppred{\code{list}}{x_0{,}n_0} {\wedge} n_0{<}0},
 \savespace\[ \savespace
\begin{array}{l}
\seppred{\code{list}}{x{,}n} ~{\equiv}~ \emp {\wedge} x{=}\nil {\wedge} n{=}0) \quad ~|~  x{=}\nil {\wedge} n{=}0\\
 \quad \quad \vee~
(\exists q{,}n_1 {\cdot}~ \sepnode{x}{node}{q{,}n_1} {\sep} \seppred{\code{list}}{q{,}n_1} {\wedge} n_1{=}n{-}1) \quad |~ x{\neq}\nil \\
\quad \invo~ \true;
\end{array}
\]
\noindent Derivation proof for this formula is presented in
Fig. \ref{fig.unfold.cyclic}.
The first branch of \code{list} has been pruned when unfolding \form{\D_0}
 as it does not satisfy the context \form{n_0{<}0}.
\form{\D_{12} {\equiv} {\exists} q_1{,}n_1 {\cdot}~ \sepnode{x_0}{node}{q_1{,}n_1} {\sep}
 \seppred{\code{list}}{q_1,n_1}  {\wedge} n_1{=}n_0{-}1 {\wedge} n_0{<}0}.
\form{\D_{12}} is linked back to \form{\D_0} as follows.
\savespace\[ \savespace
\begin{array}{lll}
1. & \sepnode{x_0}{node}{q_2{,}n_2} {\sep}
 \seppred{\code{list}}{q_2,n_2}  {\wedge} n_2{=}n_0{-}1 {\wedge} n_0{<}0 & ~~\text{refreshing existantial variables}\\
2. & \sepnode{x_3}{node}{x_0{,}n_0} {\sep}
 \seppred{\code{list}}{x_0,n_0}  {\wedge} n_0{=}n_3{-}1 {\wedge} n_3{<}0 & ~~\text{subsituting inductive variables}\\
3. & \seppred{\code{list}}{x_0,n_0}  {\wedge} n_0{<}0 & ~~\text{weakening}\\
\end{array}
\]
Thus,
  \form{\D_{12}} is marked as close and {\algonamesl} forms
a cyclic proof for \form{\D_0}.
%%\form{\sstate_{i} {=} \{ \}}, \form{\sstate {=} \{ \}}.
 {\algonamesl} returns {\unsat}.


==> cyclic-tree.tex <==
\begin{wrapfigure}{r}{0.18\textwidth}\savespace \savespace \savespace \saveone %% \savespace \saveone
\begin{center}
\caption{Cyclic.}
\begin{minipage}{0.18\textwidth} \savespace \savespace
\begin{frameit} \savespace
\begin{tikzpicture}[sibling distance=16mm, level 2/.style={sibling distance=22mm},
     level 3/.style={sibling distance=7mm},
    level distance=22pt,
  every node/.style = {align=center},
   unreach/.style     = {circle,draw,align=center,radius=2mm},
  ]]
  \node {\footnotesize $\D_0^\bigstar$}
    child [dotted] { node [unreach] {\footnotesize \underline{}} } %% $\D_{11}$
    child { node {\footnotesize $\D_{12}^\bigstar$} }
;
\end{tikzpicture}
\end{frameit}
\end{minipage}  \savespace %% \saveone
\label{fig.unfold.cyclic}
\end{center}\savespace
\end{wrapfigure}
%\end{figure}


==> deci-frag.tex <==

 as follows.
Given an inductive predicate \form{\seppredF{\code{P^N}}{\setvars{x}}}
where \setvars{x} is the sequence of \form{m} integer parameters.
Let \seppredF{\code{P^N}}{\setvars{v}_i} (\form{i \in \{1...l\}}) be any sub-term in one of its recursive branches. %% ,
%% and \form{x'_i{=}r_i{-}l'_i}.
%% Finally, let \form{\setvars{x}} and \form{\setvars{x}'}
%% be sequences of \form{k} such \form{x_i} variables.
\form{R \in Z^m {\times} Z^m} is an integer relation over
variables \form{\setvars{x}} and \form{\setvars{v}_i}, its
{\em transitive closure} is written as \form{R^+{=}\bigcup_{i{=}1}^\infty}
where \form{R^1{=}R} and \form{R^{i{+}1}{=}R^i{\circ}R}
for all \form{i{\geq}1}.
The relation \form{R} is defined as one of the  following two forms.
\begin{itemize}
\item Octagonal relation \cite{Marius:CAV:2010}.
An {\em octagonal relation} is a finite
conjunction of the form
 \form{R(x_1{,}x_2){\equiv}\underline{+} x_1 \underline{+} x_2{\leq}k}
where \form{k} is an integer constant,
\form{x_1{,}x_2 {\in} (\setvars{x} {\cup}\setvars{v}_1\cup...\cup\setvars{v}_l)}.
\scnay{Is $k$ here the same $k$ mentioned  above? If not, can we rename it?}
\item DPI relation \cite{Makoto:APLAS:2016}.
A {\em DPI relation} is a finite
conjunction of constraints of the form
 \form{R(\setvars{y}){\equiv}y_i {+} f(\setvars{z}) {\leq} k_1},
or \form{R(\setvars{y}){\equiv}y_i {+} f(\setvars{z}) {\geq} k_2}
where \form{\setvars{y} \subseteq \setvars{x} {\cup}\setvars{x}'},
\form{y_i \in \setvars{x} {\cup}\setvars{x}'},
\form{\setvars{z} \subseteq (\setvars{x} {\cup}\setvars{v}_1\cup...\cup\setvars{v}_l)},
\form{k_1} and \form{k_2} are integer numbers and
 \form{f(\setvars{z}) {\equiv} z_i ~|~ min(f(\setvars{z_1}),f(\setvars{z_2}))
~|~ max(f(\setvars{z_1}),f(\setvars{z_2}))}
\end{itemize}
Additionally, for boundedness, predicates containing
octagonal/affine relations are required to be {\em flat} (no nested loops) \cite{Ganty:TR:2016}.
For example \form{R(x_1{,}x_2){\equiv}x_1-x_2{=}5} is an octagonal relation
as it is equivalent to \form{R(x_1{,}x_2){\equiv}x_1-x_2{\leq}5 \vee x_2-x_1{\leq}-5}.
\cite{Marius:CAV:2010} and \cite{Makoto:APLAS:2016} show that
the transitive closure of these periodic relations is Presburber-definable
 and effectively computable. %% Furthermore, it is well known that
%% these Presburber-definable relations
%% are ultimately periodic.
%%The periodic set is defined as follows.
%% \begin{defn}
%% A set $S$ of integers is defined to be {\em ultimately periodic} if
%% there are some $M \ge 0$, $p > 0$ s.t.~$n \in S$ iff $n+p \in S$ for all $n \ge M$.
%% We call the set $(M,p)$-periodic.
%% \end{defn}
%% Set $(M,p)$-periodic is important for the complexity analysis.

%% \begin{defn}
%% A formula \form{\heap{\wedge}\pure}
%%  is said to be in the
%% {\slap} fragment if
%% (i) \form{\pure} is a conjunction of the above periodic relations;
%%  and (ii)
%% for every predicate \code{P} occurring in \form{\heap},
%% constraints  over
%% integer parameters in
%%  definition of \code{P} are restricted within the periodic relations defined above.
%% \end{defn}


==> ex-rec.tex <==
\begin{figure}
%% \begin{wrapfigure}{l}{0.47\textwidth}
\savespace %% \saveone
\begin{center} 
\begin{minipage}{0.45\textwidth}
\begin{frameit} \savespace % \savespace \saveone
\begin{small}\savespace \[
\begin{array}{ll}
1 & \code{int~fibo(int~n)\{} \\
2 & \code{~~ if(n{<}1)~ return~ 0;}  \\
3 & \code{~~ else~if(n{==}1)~ return~ 1;}  \\
4 & \code{~~ else~ return ~fibo(n-1){+}fibo(n-2);}  \\
5 & \code{\}} \\
%% \end{array}
%% \quad
%% \begin{array}{ll}
\\
6 & \code{int~main()\{} \\
7 & \code{~~ int(x{=}5);}  \\
8 & \code{~~ int~result{=}fibo(x);}  \\
9 & \code{~~ if(result{!=}5)~ \_\_VERIFIER\_error();}  \\
10 & \code{~~ return ~0;\}} \\
\end{array}
\] %%\savespace 
\end{small} %%\savespace \savespace 
\end{frameit}
\end{minipage} %%\savespace \saveone
\caption{fibo\_5\_true-unreach-call.c of Recursive category in SV-COMP15 competition \cite{svcomp:15}.}
\label{fig.rec}
\end{center} \saveone
\end{figure}
\hide{
\begin{verbatim}

int fibo(int n) {
    if (n < 1) {
        return 0;
    } else if (n == 1) {
        return 1;
    } else {
        return fibo(n-1) + fibo(n-2);
    }
}

pred fibo_v<n,r,e> == n<1 & r=0 & e=1
   or n=1 & r=1 & e=1
   or  _::fibo_v<n-1, r1, e1> * _::fibo_v<n-2, r2, e2> & n>1 & r=r1+r2 & e1=1 & e2=1 & e=1.

int main() {
    int x = 5;
    int result = fibo(x);
    if (result != 5) {
        __VERIFIER_error();
    }
    return 0;
}

pred main_v<r,e> ==  _::fibo_v<x,result,e_1> & x=5  & result!=5 & e_1=1 & e=0
   or  _::fibo_v<x,result,e_1> & x=5 & result=5 & e_1=1 & e=1
   or  _::fibo_v<x,result,e_1> & x=5 & e_1=0 & e=0.

checksat _::main_v<r,e> & e=0.

expect Unsat.

\end{verbatim}}


==> expr-sat-comb-fig.tex <==

\begin{table*}[thb]
% \vspace{-5pt} %%\savespace
%\begin{small}
%\scriptsize
\begin{center}
%%\begin{minipage}{16cm}
%% \vspace{-2.7mm}
%\hspace{-3.2cm} {
\begin{tabular}[t]{|c  |c |c | c| c|c|c|c|c|c|c|c}
\hline
 Data Structure (pure props) &\#queries & \multicolumn{3}{|c|}{\sleek} &
\multicolumn{3}{|c|}{\sleekplus} & \multicolumn{3}{|c|}{\algonamesl}
\\
\hline
 & & \#{\unsat} & \#{\sat}  &  sec & \#{\unsat} & \#{\sat}  &  sec & \#{\unsat} & \#{\sat}  &  sec \\
\hline
 Singly llist (size) %& 26
 & 666 &
& & & & & &
 75 & 591 & 0.67 \\ 
Even llist (size) % & 9
 & 139 &
& & & & & &
 130 & 9  & 0.33 \\ 
 Sorted llist (size, sorted%,sets
) %& 5
 & 217 &
& & & & & &
 21 & 196  & 0.51    \\
 Doubly llist (size%,sets
) %  & 5
 & 452 &
& & & & & &
 50 & 402 & 1.03  \\
 CompleteT (size, minheight) % & 5
 & 393 &
& & & & & &
 32 & 361  & 2.01  \\
 Heap trees (size, maxelem) % & 6
 & 487 &
& & & & & &
 41 & 446  &  3.75   \\
  AVL (height, size) %  &  7
 & 881  &
& & & & & &
  62 & 819  & 14.80 \\
BST (height, size, sorted) %  & 5
 &  341 &
& & & & & &
 34 & 307  & 0.99 \\
RBT (size, blackheight, color) %  & 17
 & 1741  &
& & & & & & 217 & 1524   & 10.35 \\
rose-tree  %  & 2
 &  55 & 
& & & & & &
6 & 49  & 0.04  \\
TLL %   & 2
  & 128 & 
& & & & & &
10 & 118   & 0.19   \\
 Bubble (size, sorted) % & 5
  &  300 &
& & & & & &  20 & 280   & 0.61 \\
 Quick sort (size, sorted) %,sets
  &  225 &
& & & & & &
  28 & 197   & 0.79 \\
\hline
\end{tabular}
\end{center}
\caption{Experimental Results on Wide Range of Complex Data Structures}
\label{tbl:expr:veri}
%\end{small}
\end{table*}


==> expr-sat-comb.tex <==
\input{expr-sat-comb-fig}

\locsay{to compare SLEEK, SLEEK+BAGA, S2SAT}

In the second experiment, we evaluate {\algonamesl} in the context of actual program verification. 
{\algonamesl} solver is integrated into {\hip} \cite{Chin:SCP:12,Loc:CAV:2014} system %% for deciding unsat queries
to prune infeasible program paths in symbolic execution.
Furthermore, {\algonamesl} is also used by
%% and discharge verification conditions  with SLEEK as follows.
the entailment procedure SLEEK to discharge verification conditions (VC) generated.
Specially, when SLEEK deduces a VC to the form \form{\D~ {\ent}~ \emp{\wedge}\pure_r},
SLEEK invokes {\algonamesl} to discharge the following query:
\form{\D {\wedge}\neg\pure_r}.

We evaluated {\algonamesl} deciding formulas over complex data structures in the 
compositional verification system  {\hip}.
The result is described in Table \ref{tbl:expr:veri}.
Each line shows a test on one program.
The first column lists data structures and their pure properties. %% of a program.
\code{rose{\mhyphen}trees} are trees with nodes that are allowed to have
variable number of children, stored as doubly-linked lists. %%  and \code{mcf}
%% trees are rose-tree variants where children are stored in
%% doubly-linked lists with sibling and parent pointers.
TLL is binary tree that each node points to its parent and all leave nodes
are linked as singly-linked list.
%% Definitions of these data structures and their invariants that were inferred
%% are presented in App. \ref{app.infer.inv}.
% \#Proc expresses the number procedures of each program.
\#queries is the total number of satisfiability queries sent to {\algonamesl} %% when verifying a program.
for each data structure.
The next two columns report the outputs from {\algonamesl}.
The last column shows the time taken by the \code{\algonamesl} solver.
In this experiment, {\algonamesl} terminated on all queries.
Furthermore it exactly
decided all {\sat} and {\unsat} queries.
This experimental results show that {\algonamesl} is expressive,
and can be integrated into
program verification systems for discharging  satisfiability problems
of separation logic formulas.


==> expr-sat.tex <==
\input{impl-table-sat}
%%
\locsay{to compare with SLEEK+BAGA}

We conducted an experiment on comparing performace of
{\sleek} \cite{}, {\sleekplus} \cite{},
{\slsat} \cite{} and {\algonamesl} with memorization, proof slicing and under-approximated invariants
 performance on this set of benchmarks.

\locsay{revise}
predicates of size \form{O}(n)
 and {\slsat} runs in $\Omega(2^n)$ time and space regardless of search strategies.
 The results are shown in Table \ref{tbl:expr:eff}.
The size \code{n} of \code{succ{-}circuit*} (\code{succ{-}rec*}) benchmarks expresses the breadth (depth, resp.) of dependency.

This set of benchmarks is
the User-Defined Predicate Satisfiability (UDB\_sat) suite of SL-COMP 2014
%% for Separation Logic
 \cite{smtcomp:sl:14}.
The output is either a definite answer (sat, unsat) with running time (in millisecond (ms), or second (s)), or an error. In particular,
SO denotes stack overflow; TO denotes timeout (i.e., tools run longer than 1800 seconds); and X denotes a fatal error.

\noindent{\em Results. }
The experimental results show that {\algonamesl} is much more robust and
also more efficient than {\slsat}.
While {\algonamesl} successfully solved 24 (out of 40) benchmarks, {\slsat} was capable of handling 17 benchmarks.
Furthermore, on 17 benchmarks that {\slsat} discharged successfully, {\algonamesl}
 outperforms {\slsat}, i.e., about 6.75 (3126seconds/462seconds) times faster.
As shown in the table, {\algonamesl} ran with neither stack overflow nor fatal errors over all
these challenging benchmarks.


==> expr-tbl-false.tex <==
\begin{table}[t]
% \vspace{-5pt} \savespace
%\begin{small}
%\scriptsize
\begin{center}
\caption{Experimental Results for Error Finding} %%\savespace
% \saveone %% \saveone
\label{tbl:expr:rec:false}
%%\begin{minipage}{16cm}
%% \vspace{-2.7mm}
%\hspace{-3.2cm} {
%%\begin{tabular}[t]{|c@{}|c@{}| c@{}|c@{} | c@{} | c@{}  | c@{} | c@{}| c@{}|}
\begin{tabular}[t]{|c|c| c |c | c | c | c  | c|}
\hline
\multirow{2}{3em}{Tool} & \multicolumn{6}{|c|}{Safety Verification}\\
\cline{2-7}
  & e$\surd$ & e\ding{55} &  unk & TO &  points & time \\
\hline
%%BLAST \cite{Henzinger:2002:POPL} & & & & & & & \\
%%Symbiotic \cite{Chalupa:TACAS:2016}  &   &  &  &   &  &  \\
%%Map2Check \cite{Herbert:SEFM:2015}  &   &  &  &    &  &  \\
{ PredatorHP\cite{Predator:SV:16}}   &  &  &  &  & &  \\
{ Cascade \cite{Wei:VMCAI:2014}}  & 8 & 0  & 50  & 4  & 8 & 13m5s \\
{ SeaHorn \cite{Gurfinkel:CAV:2015}} &  &  &  &  & & \\
{ ESBMC \cite{Cordeiro:2011:ICSE}} &   &  &  &  &  & \\
{ UAutomizer \cite{Heizmann:CAV:13}} &  &  &  &  &  & \\
{ CPA-Seq \cite{Beyer:CAV:2007}}  &  47 & 4 & 1 & 10 & {-}81 & 25m36s\\
{ CBMC \cite{Clarke:TACAS:2004}} & 51 & 2 & 0 & 9  & {-}13  & 28m45s \\
%% PAC-MAN\cite{DBLP:journals/corr/ChenHLLTWW15} & & & & & & & \\
{ Smack-Corral \cite{Haran:TACAS:2015}}  &   &   & &  &  &  \\
{\bf \toolname}  & {\bf59} & {\bf 0} & {\bf 0} & {\bf 3} & {\bf 58 }  &  {\bf 10m36s }  \\
\hline
\end{tabular}%\saveone
\end{center}
%\end{small}
\end{table}


==> expr-tbl-true.tex <==
\begin{table}[t]
% \vspace{-5pt} \savespace
%\begin{small}
%\scriptsize
\begin{center}
\caption{Experimental Results for Safety Verification} %%\savespace
% \saveone %% \saveone
\label{tbl:expr:rec:true}
%%\begin{minipage}{16cm}
%% \vspace{-2.7mm}
%\hspace{-3.2cm} {
%%\begin{tabular}[t]{|c@{}|c@{}| c@{}|c@{} | c@{} | c@{}  | c@{} | c@{}| c@{}|}
\begin{tabular}[t]{|c|c| c | c | c | c  | c|}
\hline
Tool &  s$\surd$ &  s\ding{55} & unk & TO &  points & time\\
\hline
%%BLAST \cite{Henzinger:2002:POPL} & & & & & & & \\
%%Symbiotic \cite{Chalupa:TACAS:2016}  &   &  &  &   &  &  \\
%%Map2Check \cite{Herbert:SEFM:2015}  &   &  &  &    &  &  \\
{PredatorHP\cite{Predator:SV:16}}   &  &  & &  &  &  \\
{Cascade \cite{Wei:VMCAI:2014}}  &  0 & 0 & 58 & 16 &  0 & 48m45s \\
{SeaHorn \cite{Gurfinkel:CAV:2015}} &  &  & & &  &  \\
{ESBMC \cite{Cordeiro:2011:ICSE}}  &  &  &  & &  &  \\
{UAutomizer \cite{Heizmann:CAV:13}} &   &  & & &  &  \\
{CPA-Seq \cite{Beyer:CAV:2007}}   & 54  &  0 & 4 &  16 & 108 &  51m41s \\
{CBMC \cite{Clarke:TACAS:2004}}  & 35  & 0 & 0 & 39 & 70 & 130m29s \\
%% PAC-MAN\cite{DBLP:journals/corr/ChenHLLTWW15} & & & & & & & \\
{Smack-Corral \cite{Haran:TACAS:2015}}  &   & &  &  &  &  \\
{\bf \toolname}  & {\bf 59} & {\bf 0} & {\bf 1} &  {\bf 14}& {\bf 120} & {\bf 44m40s}  \\
\hline
\end{tabular}%\saveone
\end{center}
%\end{small}
\end{table}


==> expr-tbl.tex <==
\begin{table}[t]
% \vspace{-5pt} \savespace
%\begin{small}
%\scriptsize
\begin{center}
\caption{Experimental Results} %%\savespace
% \saveone %% \saveone
\label{tbl:expr:rec}
%%\begin{minipage}{16cm}
%% \vspace{-2.7mm}
%\hspace{-3.2cm} {
%%\begin{tabular}[t]{|c@{}|c@{}| c@{}|c@{} | c@{} | c@{}  | c@{} | c@{}| c@{}|}
\begin{tabular}[t]{|c|c| c |c | c | c  | c | c| c|}
\hline
Tool &  s$\surd$ & e$\surd$ & unk & s\ding{55} & e\ding{55}   & pts & mins\\
\hline
%%BLAST \cite{Henzinger:2002:POPL} & & & & & & & \\
%%Symbiotic \cite{Chalupa:TACAS:2016}  &   &  &  &   &  &  \\
%%Map2Check \cite{Herbert:SEFM:2015}  &   &  &  &    &  &  \\
{\small PredatorHP\cite{Predator:SV:16}}  & 37  & 46 & 35 & 14 & 0 & -104 & 49 \\
{\small Cascade \cite{Wei:VMCAI:2014}}  & 0  & 8 & 124 & 0 & 0 &  8  & 50 \\
{\small SeaHorn \cite{Gurfinkel:CAV:2015}} & 59 & 58 & 5 & 10 & 0 & 16 & 19 \\
{\small ESBMC \cite{Cordeiro:2011:ICSE}} &  36 & 41 & 52 & 0 & 3  & 17 & 115 \\
{\small UAuto \cite{Heizmann:CAV:13}} & 27 & 30 & 75 & 0 & 0 & 84 & 113 \\
{\small CPA-Seq \cite{Beyer:CAV:2007}}  &  54 & 46 & 31 & 0 & 1 & 122 & 79 \\
{\small CBMC \cite{Clarke:TACAS:2004}} & 44 & 51 & 36 & 1 & 0 & 123  & 142 \\
%% PAC-MAN\cite{DBLP:journals/corr/ChenHLLTWW15} & & & & & & & \\
{\small Smack-Corral \cite{Haran:TACAS:2015}} & 44 & 50 & 38   & 0  & 0 & 138 & 125 \\
{\bf \toolname}  & {\bf 59} & {\bf 57} & {\bf 16} & {\bf 0} & {\bf 0} & {\bf 175} & {\bf 38}  \\
\hline
\end{tabular}%\saveone
\end{center}
%\end{small}
\end{table}


==> expr-witness.tex <==

While {\toolname} is sound for both verifying and falsifying, 
it is not necessary to validate
the counterexample.
In this experiment, we show that  error witnesses generated by {\toolname}
are correct; they are can be validated by validators, e.g. CPAChecker
\cite{Dirk:CAV:2015}.
However, CPAChecker has not supported the validation for the
errors of heap-manipulating programs. As such,
we conduct the experiment on C recursive programs taken from
Recursive subcategory of SV-COMP \footnote{http://sv-comp.sosy-lab.org/2016/}.
In this set of benchmarks, there are ... error problems.
%%\noindent {\em Benchmark Set.}

\locsay{to revise}

\noindent{\em Results. } all error witnesses generated by our tool
were validated by  CPAChecker.


==> fix-ex.tex <==
For illustration, consider satisfiability check of the formula:
 \form{\D_0 {\equiv} \seppred{\code{Q}}{x_0,y_0} {\wedge}
 x_0{=}y_0 {\wedge} x_0{\neq}\nil}, whereas
 \savespace\[ \savespace
\begin{array}{l}
\seppred{\code{Q}}{x{,}y} ~{\equiv}~ (\exists c{,}d {\cdot}~ \emp {\wedge}
            y{=}\nil {\wedge} x{\neq}\nil) \quad ~|~  y{=}\nil {\wedge} x{\neq}\nil\\
\quad \quad  \vee~
(\exists c {\cdot}~ \seppred{\code{Q}}{x{,}c} {\wedge} y{\neq}\nil) \quad~~ |~ y{\neq}\nil 
\qquad \invo~ \true;
\end{array}
\]
\noindent Derivation proof for this formula is presented in Fig. \ref{fig.unfold.fix}
\form{\D_{12} {\equiv} \exists c_2{,}d_2 {\cdot}~ \seppred{\code{Q_2}}{x_0,c_2}
  {\wedge} y_0{\neq}\nil}
 \form{{\wedge} x_0{=}y_0 {\wedge} x_0{\neq}\nil }.
(The first branch of \code{Q} has been pruned when unfolding \form{\D_0} as it does not satisfy the context \form{x_0{=}y_0}).
Since \code{\fix} could link \form{\D_{12}}
 back to \form{\D_0},
  \form{\D_1} is marked as close.
Thus  \form{\sstate_{i} {=} \{ \}}, \form{\sstate {=} \{ \}}.
Consequently, {\algoname} returns {\unsat}.


==> fix-tree.tex <==
\begin{wrapfigure}{r}{0.18\textwidth}\savespace \savespace \savespace \savespace
\begin{center}
\caption{Fixpoint.}
\begin{minipage}{0.18\textwidth} \savespace \savespace
\begin{frameit} \savespace
\begin{tikzpicture}[sibling distance=16mm, level 2/.style={sibling distance=22mm},
     level 3/.style={sibling distance=7mm},
    level distance=22pt,
  every node/.style = {align=center},
   unreach/.style     = {circle,draw,align=center,radius=2mm},
  ]]
  \node {\footnotesize $\D_0$}
    child [dotted] { node [unreach] {\footnotesize \underline{}} } %% $\D_{11}$
    child { node {\footnotesize $\D_{12}$} }
;
\end{tikzpicture}
\end{frameit}
\end{minipage}  \savespace %% \saveone
\label{fig.unfold.fix}
\end{center}\savespace
\end{wrapfigure}
%\end{figure}


==> impl-table-sat.tex <==
\begin{table*}[t]
% \vspace{-5pt} %%\savespace
%\begin{small}
%\scriptsize
\begin{center}
\caption{Worst-Case Complexity Satisfiability Checks}
\label{tbl:expr:eff}
%%\begin{minipage}{16cm}
%% \vspace{-2.7mm}
%\hspace{-3.2cm} {
\begin{tabular}[t]{|c|c| c|c|c|c|c|c|c|c|}
\hline
n &
\multicolumn{3}{|c|}{abduced (1-20)}
&
 \multicolumn{3}{|c|}{succ-circuit (1-20)}
 & \multicolumn{3}{|c|}{succ-rec (1-20)}
\\
\hline
   & {\sleekplus} & {\slsat}       & {\algonamesl} & {\sleekplus} & {\slsat}      & {\algonamesl} & {\sleekplus} & {\slsat}   & {\algonamesl}   \\
\hline
1 &  & & &   & 1 ms     &  21 ms      &  & 0 ms     & 25 ms       \\
2 &  & & &   & 2 ms     &  23 ms      &  & 1 ms     & 30 ms       \\
3 &  & & &   & 27 ms    &  30 ms      &  & 4 ms     & 33 ms      \\
4 &  & & &   & 867ms    &  34 ms      &  &  21 ms    & 39 ms        \\
5 &  & & &   & 30 s     &  0.05 s     &  &  134 ms   & 52 ms      \\
6 &  & & &   & 30 s     &  0.09 s     &  &  830 ms   & 76 ms      \\
7 &  &  & &  & SO       &  0.20 s     &  & 5.0 s    & 0.21 s      \\
8 &  & & &  & SO       &  0.61 s     &   & 29.5 s   &  0.87 s    \\
9 &  & & &  & SO       &  2.21 s     &   & 167.8 s  &  4.83 s   \\
10 & & & &  & SO       &  8.49 s    &    & 1065 s   & 45.28 s  \\
11 & & & &  & SO       &  37.46 s   &    & 1796.4 s & 410.92 s \\
12 & & & &  & SO       &  170.53s   &    & TO       & TO \\
13 & & & &  & SO       &  988.29s   &    & TO       & TO \\
14 & & & &  & SO       &  TO         &   & X        & TO \\
15 & & & &  & SO       &  TO        &    & X        & TO \\
16 & & & &  & SO       &  TO        &    & X        & TO \\
17 & & & &  & SO       &  TO        &    & X        & TO \\
18 & & & &  & SO       &  TO        &    & X        & TO \\
19 & & & &  & SO       &  TO        &    & X        & TO \\
20 & & & &  & SO       &  TO        &    & X        & TO\\
\hline
\end{tabular}
\end{center}
\savespace 
%\end{small}
\end{table*}



==> more-ex.tex <==
\begin{figure}[tb]
\begin{center}
\begin{minipage}{0.47\textwidth} 
\begin{frameit} \savespace \savespace
\[
\begin{array}{ll}
1. & \code{foo(node~x)}\\
  & \form{PRE: \emp{\wedge}\dangl{x'}} \\
2. & \code{~~~\{int~v = x{\der}val;} \\
 & \form{// \D_1 \vee \D_2 \vee \D_3} \\
3. & \code{~~~~assume(false);\}} \\
  & \form{// \D_1 \vee \D_2 \vee \D'_3} \\
& \text{a)}
\end{array}
\]
\end{frameit}
\end{minipage}
\caption{Halt for Error}\label{fig.examples}
\end{center}
\end{figure}

\begin{figure}[tb]
\begin{center}
\begin{minipage}{0.47\textwidth} 
\begin{frameit} \savespace \savespace
\[
\begin{array}{cc}
\begin{array}{l}
1. \code{hoo1(node~x, node~y)}\\
   \form{PRE: \sepnodeF{x}{_}{v,\nil}{\wedge}\dangl{y'}} \\
2. \code{\{~~~assume(x{=}y);}\\
  \form{\quad// \D_4} \\
3.  \code{~~~~int~i{=}y{\der}val;}\}\\
  \form{\quad// \D_5 \vee \D_6 \vee \D_7} \\
 \text{b)}
\end{array}
&
\begin{array}{l}
1. \code{hoo2(node~x, node~y)}\\
   \form{PRE: \sepnodeF{x}{_}{v,\nil}{\wedge}\dangl{y'}} \\
2. \code{\{~~~int~i{=}y{\der}val;}\\
  \form{\quad // \D_8 \vee \D_9 \vee \D_{10}} \\
3. \code{~~~~assume(x{=}y);}\}\\
  \form{\quad// \D_8 \vee \D_9 \vee \D'_{10}} \\
 \text{c)}
\end{array}
\end{array}
\]
\end{frameit}
\end{minipage}
\caption{Flow-Sensitive Encoding}\label{fig.flow.examples}
\end{center}
\end{figure}

\begin{figure}[tb]
\begin{center}
\begin{minipage}{0.45\textwidth} 
\begin{frameit} \savespace \savespace
\[
\begin{array}{cc}
\begin{array}{l}
 \code{goo1(node~x)}\\
 \form{PRE: \emp{\wedge}\dangl{x'}} \\
 \code{~~~\{x{=}alloca()}\\
 \code{~~~~del(x);}\}\\
%& \text{a)}
\end{array}
&
\begin{array}{l}
 \code{goo2(node~x)}\\
 \form{PRE: \emp{\wedge}\dangl{x'}} \\
 \code{~~~\{del(x);}\\
 \code{~~~~x{=}alloca();\}}\\
%& \text{b)}
\end{array}
\end{array}
\]
\end{frameit}
\end{minipage}
\caption{Inter-procedural Encoding}\label{fig.inter.examples}
\end{center}
\end{figure}

In the following, we illustrate three examples
in Fig. \ref{fig.examples}, Fig. \ref{fig.flow.examples}
 and  Fig. \ref{fig.inter.examples}
to emphasize that our system never generates any infeasible
execution. The program in Fig. \ref{fig.examples}a)
triggers a null-deference error at line 2.
The post-states at line 2 is \form{\D_1\vee\D_2\vee\D_3}
where
\[
\form{\D_1{\equiv}\emp{\wedge}\dangl{x'}{\wedge} x'{=}null {\wedge}\error{=}1 }, \form{\D_2{\equiv}\emp{\wedge}\dangl{x'}{\wedge} \dangl{x'} {\wedge}\error{=}1 }
\]
and
\[ \form{\D_3{\equiv}\emp{\wedge}\dangl{x'}{\wedge}  x'{\neq}null
{\wedge}\neg\dangl{x'} {\wedge} \sepnodeR{x'}{val}{v'}{0}}
\]

As \form{\D_1} and \form{\D_2} contains errors, the symbolic execution over these two branches halts.
Thus, only \form{\D_3} branch is forwarded for the execution at
line 3
and its post-state
\[ \form{\D'_3{\equiv}\emp{\wedge}\dangl{x'}{\wedge}  x'{\neq}null
{\wedge}\neg\dangl{x'} {\wedge} \sepnodeR{x'}{val}{v'}{0}{\wedge}\false}
\]
Since our decision procedure detects that
\form{\D_1} and \form{\D_3'} are \form{\false}
and \form{\D_2} is a satisfiable error formula,
it properly concludes that this program has an error.

We use two programs in Fig. \ref{fig.flow.examples}
to illustrate the flow-sensitive encoding.
We swap statements at lines 2-3.
While \code{hoo1} is safe,
\code{hoo2} is erroneous at line 2.
For \code{hoo1}, the proposed executor
generates the following states.
\[
\begin{array}{l}
\D_4{\equiv}\sepnodeF{x'}{_}{v,\nil}{\wedge}\dangl{y_1}{\wedge}x'{=}y'\\
\D_5{\equiv}\exists i.~\sepnodeF{x'}{_}{v,\nil}{\wedge}\dangl{y_1}{\wedge}x'{=}y'{\wedge}\dangl{y'}{\wedge}\error{=}1 \\
\D_6{\equiv}\exists i.~\sepnodeF{x'}{_}{v,\nil}{\wedge}\dangl{y_1}{\wedge}x'{=}y'{\wedge}y'{=}\nil{\wedge}\error{=}1 \\
\D_7{\equiv}\exists i.~\sepnodeF{x'}{_}{v,\nil}{\wedge}\dangl{y_1}{\wedge}x'{=}y'{\wedge}\neg \dangl{y'} {\wedge} y'{\neq}\nil{\wedge}i{=}v\\
\end{array}
\]

As our decision procedure detects that \form{\D_5}
and \form{\D_6} are \form{\false},
and \form{\D_7} is not an error formula,
 our system concludes that
\code{hoo1} is safe.

For \code{hoo2}, the proposed executor
generates the following states.
\[
\begin{array}{l}
\D_8{\equiv}\exists i.~\sepnodeF{x'}{_}{v,\nil}{\wedge}\dangl{y'}{\wedge}\dangl{y'}{\wedge}\error{=}1 \\
\D_9{\equiv}\exists i.~\sepnodeF{x'}{_}{v,\nil}{\wedge}{\wedge}\dangl{y'}y'{=}\nil{\wedge}\error{=}1 \\
\D_{10}{\equiv}\exists i.~\sepnodeF{x'}{_}{v,\nil}{\wedge}\dangl{y'}{\wedge}\neg \dangl{y'} {\wedge} y'{\neq}\nil{\wedge}i{=}v\\
\D'_{10}{\equiv}\exists i.~\sepnodeF{x'}{_}{v,\nil}{\wedge}\dangl{y_1}{\wedge}\neg \dangl{y_1} {\wedge} y_1{\neq}\nil{\wedge}i{=}v{\wedge}x'{=}y'\\
\end{array}
\]

As our decision procedure detects that \form{\D_8}
is a satisfiable error formula
(and \form{\D_9} and  
and \form{\D'_{10}} are \form{\false}),
 our system concludes that
\code{hoo2} has an error.

Finally, for those programs in Fig. \ref{fig.inter.examples},
 while function \code{alloca} allocates
and returns a new node,
function \code{del} de-allocates the node pointed-to by
the parameter.
Our executor encodes these program as follows.
\[
\begin{array}{l}
\defpred~\form{\seppred{goo1}{x,\res{,}\error}} ~\equiv~
\form{alloca(x,\_)^0_0 {\sep} del(x,\error)^1_0 {\wedge}\dangl{x} } {:}[1]
\end{array}
\]

\[
\begin{array}{l}
\defpred~\form{\seppred{goo2}{x,\res{,}\error}} ~\equiv~
del(x,\error)^0_0{\sep}\form{alloca(x,\_)^1_0 {\wedge}\dangl{x} } {:}[1]
\end{array}
\]

As can be seen, the main different between definitions of
predicates
\form{goo1} and \form{goo2} is the sequence numbers
annotated for predicates \form{alloca}
and \form{del}.
Our decision procedure always follows
these numbers to unfold predicates \form{alloca}
and \form{del}. Thus, for \form{goo1} 
predicate \form{alloca} is unfolded before \form{del},
 no error in \form{goo1}.
For \form{goo2} 
predicate \form{del} is unfolded first, and
our decision procedure detect  an error.


==> mov-leak.tex <==
\[
\begin{array}{l}
\form{\D_{51}{\equiv} x{=}\nil {\wedge} n_0{=}0 {\wedge}\error_1{=}0
{\wedge} \seppred{inv_{12}}{x{,}x'{,}\error_2}_{1}^1 {\wedge}n_0{\geq}0 } \\
\quad  \form{{\wedge}\error_1{=}0 {\wedge}\error_2{=}0 {\wedge}\error_0{=}1\nemp} \\
%
\form{\D_{52}{\equiv} \sepnode{x}{node}{n_1{,}r_2} {\sep}
\seppred{sll}{n_1{,}r_2{,}\error_1}_{2}^0 {\sep}\seppred{inv_{12}}{x{,}x'{,}\error_2}_{1}^1}\\
\quad \form{ {\wedge}n_0{\neq}0{\wedge} n_1{=}n_0{-}1
 {\wedge}n_0{\geq}0 
{\wedge}\error_1{=}0 {\wedge}\error_2{=}0 {\wedge}\error_0{=}1\nemp} \\
%% $\utree{6}$ 
\form{\D_{61}{\equiv} \underline{\emp} {\wedge} x{=}\nil {\wedge} n_0{=}0 {\wedge}\error_1{=}0
{\wedge} 
x{=}\nil  {\wedge}x'{=}x {\wedge} }\\
\quad \form{{\error_2{=}0} {\wedge}n_0{\geq}0 
{\wedge}\error_1{=}0 {\wedge} \underline{\error_2{=}0} {\wedge} \error_0{=}1\underline{\nemp}} \\
%
\form{\D_{62}{\equiv} {x{=}\nil} {\wedge} n_0{=}0 {\wedge}\error_1{=}0
{\wedge}
{\dangl{x}} {\wedge} x{\neq}\nil  {\wedge} \underline{\error_2{=}1}
 {\wedge} } \\
\quad \form{n_0{\geq}0{\wedge}\error_1{=}0 {\wedge} \underline{\error_2{=}0} {\wedge}\error_0{=}1\nemp} \\
%
\form{\D_{63}{\equiv} \underline{x{=}\nil} {\wedge} n_0{=}0 {\wedge}\error_1{=}0
{\wedge}
 {\neg}\dangl{x}
  {\wedge}\underline{x{\neq}\nil} 
{\wedge}  }\\
\quad \form{ \sepnodeR{x}{val}{v_1}{0}{\wedge}   %% v_1{=}x.val
v_1{<}0{\wedge} \error_2{=}1
 {\wedge}n_0{\geq}0 }
  \form{{\wedge}\error_1{=}0 {\wedge}} \\
\form{\quad \error_2{=}0 {\wedge}\error_0{=}1\nemp}
 \end{array}
 \]
\[
 \begin{array}{l}
%
\form{\D_{64}{\equiv} \underline{x{=}\nil} {\wedge} n_0{=}0 {\wedge}\error_1{=}0
{\wedge}
\seppred{inv_{12}}{x_1{,}x'{,}\error_2}_{2}^0{\wedge}{\neg}\dangl{x}
  {\wedge} }\\
\quad \form{\underline{x{\neq}\nil}{\wedge} \sepnodeR{x}{val}{v_1}{0} %% v_1{=}x.val
{\wedge}v_1{\geq}0{\wedge} \sepnodeR{x}{next}{x_1}{0} %% x_1{=}x.next
 {\wedge}}\\
\quad \form{n_0{\geq}0
{\wedge}\error_1{=}0 {\wedge}\error_2{=}0 {\wedge}\error_0{=}1\nemp} \\
%% \end{array}
%% \]
%% $\utree{7}$ 
%% \[
%% \begin{array}{l}
\form{\D_{71}{\equiv} \underline{\sepnode{x}{node}{n_1{,}r_2}} {\sep}
\seppred{sll}{n_1{,}r_2{,}\error_1}_{2}^0
{\wedge} \underline{x{=}\nil}  {\wedge}x'{=}x}\\
\quad \form{ {\wedge} {\error_2{=}0}
 {\wedge}n_0{\neq}0{\wedge} n_1{=}n_0{-}1
 {\wedge}n_0{\geq}0 
{\wedge}\error_1{=}0 {\wedge}{\error_2{=}0} {\wedge}\error_0{=}1\nemp} \\
\form{\D_{72}{\equiv} {\sepnode{x}{node}{n_1{,}r_2}} {\sep}
\seppred{sll}{n_1{,}r_2{,}\error_1}_{2}^0 {\wedge}
{{\dangl{x}}{\wedge} x{\neq}\nil }
}\\
\quad \form{ {\wedge} \underline{\error_2{=}1} {\wedge}n_0{\neq}0{\wedge} n_1{=}n_0{-}1
 {\wedge}n_0{\geq}0 
{\wedge}\error_1{=}0 {\wedge} \underline{\error_2{=}0} {\wedge}\error_0{=}1\nemp} \\
%
\form{\D_{73}{\equiv} \sepnode{x}{node}{n_1{,}r_2} {\sep}
\seppred{sll}{n_1{,}r_2{,}\error_1}_{2}^0
 {\wedge}
{\neg}\dangl{x}
  {\wedge}x{\neq}\nil {\wedge}}\\
\quad \form{ \sepnodeR{x}{val}{v_1}{0} %% v_1{=}x.val
{\wedge}v_1{<}0{\wedge}
\underline{\error_2{=}1}{\wedge}n_0{\neq}0{\wedge} n_1{=}n_0{-}1
}\\
\quad \form{ 
 {\wedge}n_0{\geq}0 
{\wedge}\error_1{=}0 {\wedge}\underline{\error_2{=}0} {\wedge}\error_0{=}1\nemp} \\
%% \form{\D_{73}{\equiv} \sepnode{x}{node}{n_1{,}r_2} {\sep}
%% \seppred{sll}{n_1{,}r_2{,}\error_1}_{2}^0
%%  {\sep}
%% {\neg}\dangl{x} {\sep}\seppred{inv_{12}}{x_1{,}x'{,}\error_2}_{2}^1
%% }\\
%% \quad \form{ {\wedge}x{\neq}\nil {\wedge} x_1{=}x.next{\wedge}n_0{\neq}0{\wedge} n_1{=}n_0{-}1
%%  {\wedge}n_0{\geq}0 }\\
%% \quad \form{
%% {\wedge}\error_1{=}0 {\wedge}\error_2{=}0 {\wedge}\error_0{=}1\nemp} \\
\form{\D'_{74}{\equiv} \norm{\D_{73}} {\equiv}\sepnode{x}{node}{n_1{,}r_2} {\sep}
\seppred{sll}{n_1{,}r_2{,}\error_1}_{2}^0
  {\sep}
}\\
\quad \form{\seppred{inv_{12}}{r_2{,}x'{,}\error_2}_{2}^1 {\wedge}x{\neq}\nil
{\wedge}n_1{\geq}0{\wedge}n_0{\neq}0{\wedge} n_1{=}n_0{-}1
 {\wedge} }\\
\quad \form{n_0{\geq}0
{\wedge}\error_1{=}0 {\wedge}\error_2{=}0 {\wedge}\error_0{=}1\nemp} \\
\end{array}
\]


==> note <==

call-by-value, ignore the affect of mutation at calling site
func P(x)
  ==> P(x_in, x_out) == ... x_out = x_in

call-by-reference: take the affect of mutation into account at calling site
func P(ref x)
  ==> P(x_in, x_out) == ... x_out = x

function call
func Q(x) { ...P(x)..} === \Delta subst[x_fresh/x; x_out/x]* P(x, x_out) ...

==> proof-ex-elim.tex <==
While Lemma \ref{lem.elim.sound} states the ``if'' direction,
Lemma \ref{lem.elim.complete} states the ``only if'' direction.

\begin{lemma}\label{lem.elim.sound}
Let \form{\exists\setvars{w}{\cdot}\alpha} be a (dis)equality conjunction. If
\form{\sstack \force \atom} then \form{\sstack \force \projectpsh{\atom}{\setvars{w}}} 
\end{lemma}
\begin{proof}
We prove lemma \ref{lem.elim.sound} by induction on
size of \form{\atom}. The proof for this lemma is based on
semantics of \form{\wedge}.
\begin{itemize}
\item Case \form{\atom{\equiv}\true}. Trivially.
\item Case \form{\atom{\equiv}v_1{=}v_2{\wedge}\atom_1} and %%\form{v_2\in\setvars{w}},
\form{v_1\in\setvars{w}}.
\[
\begin{array}{ll}
 & \form{\sstack \force \atom} \\
\Longleftrightarrow & \form{\sstack \force v_1{=}v_2} \text{ and } 
\form{\sstack \force \atom_1} ~~(\text{semantics of } \wedge)\\
\Longrightarrow & \form{\sstack \force \atom_1[v_2/v_1]}\\
\end{array}
\]
\item Case \form{\atom{\equiv}v_1{=}v_2{\wedge}\atom_1} and \form{v_1\not\in\setvars{w}},
\form{v_2\in\setvars{w}}.
\[
\begin{array}{ll}
 & \form{\sstack \force \atom} \\
\Longleftrightarrow & \form{\sstack \force v_1{=}v_2} \text{ and } 
\form{\sstack \force \atom_1} ~~(\text{semantics of } \wedge)\\
\Longrightarrow & \form{\sstack \force \atom_1[v_1/v_2]}\\
\end{array}
\]
\item Other cases are similar
\end{itemize}
\end{proof}

\begin{lemma}\label{lem.elim.complete}
Let \form{\exists\setvars{w}{\cdot}\alpha} be a {\em satisfiable}
 (dis)equality conjunction. If
\form{\sstack \force \projectpsh{\atom}{\setvars{w}}}
\form{\exists \sstack' {\cdot} \sstack \subseteq  \sstack' \text{ and }  \sstack' \force \atom}
\end{lemma}

\begin{proof}
By induction on size of \form{\atom}.
\begin{enumerate}
\item Case \form{\atom{\equiv}\true}. Trivially.
\item Case \form{\atom{\equiv}v_1{=}v_2{\wedge}\atom_1} and \form{v_1\in\setvars{w}}.
%%\form{v_2\in\setvars{w}}.

By assumption, %%\form{\sstack \force v_1{=}v_2} (1) and
 \form{\sstack \force \projectpsh{\atom_1}{\setvars{w}}}. 
By induction, there exists a stack \form{\sstack_1} such that
\form{\sstack \subseteq \sstack_1} and
\form{\sstack_1 \force {\atom_1}}.
We examines four subcases:
\begin{enumerate}
\item Case \form{\sstack_1(v_1)} and \form{\sstack_2(v_2)} are both defined. Never.
\item Case \form{\sstack_1(v_1)} is defined and \form{\sstack_1(v_2)} is undefined.
 We define  \form{\sstack_2(v_2)} such that \form{\sstack_2(v_2){=}\sstack_1(v_1)}.
This implies  \form{\sstack_1\cup\sstack_2 \force v_1{=}v_2}.
Thus, \form{(\sstack_1\cup\sstack_2) \force \atom}.
\item Case \form{\sstack_1(v_2)} is defined, \form{\sstack_1(v_1)} is undefined
and both are undefined are similar.
\end{enumerate}
\item Case \form{\atom{\equiv}v_1{=}v_2{\wedge}\atom_1} and \form{v_1\not\in\setvars{w}},
\form{v_2\in\setvars{w}}.

By assumption, %%\form{\sstack \force v_1{=}v_2} (3) and
 \form{\sstack \force \projectpsh{\atom_1}{\setvars{w}}}. 
By induction, there exists a stack \form{\sstack_1} such that
\form{\sstack \subseteq \sstack_1} and
\form{\sstack_1 \force \atom_1 }.
We examines two subcases:
\begin{enumerate}
\item Case \form{\sstack_1(v_1)} is defined.
As \form{v_2\in\setvars{w}}, \form{v_2} has been substituted already. Thus,
\form{\sstack_1(v_2)} is undefined.
We define  \form{\sstack_2(v_2)} such that
\form{\sstack_2(v_2){=}\sstack_1(v_1)}.
This implies  \form{\sstack_1\cup \sstack_2 \force v_1{=}v_2}.
Thus, \form{(\sstack_1\cup\sstack_2) \force \atom}.
\item Case \form{\sstack_1(v_1)} is undefined.
 Never.
\end{enumerate}
%%\item Case \form{\atom{\equiv}v_1{=}v_2{\wedge}\atom_1} and \form{v_1\not\in\setvars{w}},
%%\form{v_2\in\setvars{w}}. Similar to Case 3.
\item Case \form{\atom{\equiv}v_1{=}v_2{\wedge}\atom_1} and \form{v_1\not\in\setvars{w}},
\form{v_2\not\in\setvars{w}}.
By assumption, \form{\sstack \force \projectpsh{\atom_1}{\setvars{w}}}. 
By induction, there exists a stack \form{\sstack_1} such that
\form{\sstack \subseteq \sstack_1} and
\form{\sstack_1 \force {\atom_1}}.
As  \form{v_1\not\in\setvars{w}} and
\form{v_2\not\in\setvars{w}}, \form{\sstack_1(v_1)} and \form{\sstack_1(v_2)} are both defined.
As \form{\atom} is satisfiable, \form{\sstack_1(v_1){=}\sstack_1(v_2)}.
This implies \form{\sstack_1 \force v_1{=}v_2}.
Thus,  \form{\sstack_1 \force \atom}.
\item Case \form{\atom{\equiv}v_1{\not=}v_2{\wedge}\atom_1} and \form{v_1\in\setvars{w}},
\form{v_2\in\setvars{w}}.

By assumption, \form{\sstack \force \projectpsh{\atom_1}{\setvars{w}}}. 
By induction, there exists a stack \form{\sstack_1} such that
\form{\sstack \subseteq \sstack_1} and
\form{\sstack_1 \force {\atom_1}}.
As \form{v_1\in\setvars{w}} and
\form{v_2\in\setvars{w}}, \form{\sstack_1(v_1)} and \form{\sstack_2(v_2)} are both undefined.
We define  \form{\sstack_2(v_1)} and \form{\sstack_2(v_2)} such that \form{\sstack_2(v_2){\not=}\sstack(v_2)}
(As domain of integer is infinite, we always find a such value for \form{v_1} and \form{v_2})
This implies  \form{\sstack_1 \cup \sstack_1 v_1{\not=}v_2}.
Thus, \form{(\sstack_1\cup\sstack_2) \force \atom}.
\item Case \form{\atom{\equiv}v_1{\not=}v_2{\wedge}\atom_1} and \form{v_1\in\setvars{w}},
\form{v_2\not\in\setvars{w}}. Similar to Case 5.

\item Case \form{\atom{\equiv}v_1{=}v_2{\wedge}\atom_1} and \form{v_1\not\in\setvars{w}},
\form{v_2\in\setvars{w}}. Similar to Case 5.
\item Case \form{\atom{\equiv}v_1{=}v_2{\wedge}\atom_1} and \form{v_1\not\in\setvars{w}},
\form{v_2\not\in\setvars{w}}.
By assumption, \form{\sstack \force \projectpsh{\atom_1}{\setvars{w}}}. 
By induction, there exists a stack \form{\sstack_1} such that
\form{\sstack \subseteq \sstack_1} and
\form{\sstack_1 \force {\atom_1}}.
As  \form{v_1\not\in\setvars{w}} and
\form{v_2\not\in\setvars{w}}, \form{\sstack_1(v_1)} and \form{\sstack_1(v_2)} are both defined.
As \form{\atom} is satisfiable, \form{\sstack_1(v_1){\not=}\sstack_1(v_2)}.
This implies \form{\sstack_1 \force v_1{\not=}v_2}.
Thus,  \form{\sstack_1 \force \atom}.
\end{enumerate}
\end{proof}


==> sat-algo.tex <==
 \begin{algorithm}[t]
%%\begin{procedure}
  \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
  \SetAlgoLined

 \Input{($\D${:}[])} \Output{{(\sat, $\xi$)} or {\unsat}}
   $\utree{} {\leftarrow} (\D {:}[]) $% \text{build the unfolding tree with only the root node} 
\tcc*{initialize root}

%% \While { $i<=bound$ }
  \While { $\true$ }
 {
    (\code{is\_error},\utree{}) {$\leftarrow$} \code{\uosl}(\utree{})% \hfill \text{mark any leaf node of the tree satisfiable if it is proven so}
 \tcc*[r]{base case}

   {\bf if} {\code{is\_error}} {\bf then }
   {\Return{(${\sat}$, \code{get\_error}(\utree{}))}}; %% \tcc*{\sat}}

%  \Else{
     $\utree{} {\leftarrow} \code{\oosl}(\utree{})$
% \hfill \text{mark any leaf node of the tree unsatisfiable if it is proven so}
\tcc*[r]{prune infeasible}

      $ \utree{}  {\leftarrow} \code{\lbsl}(\utree{}) $
% \hfill \text{check if any leaf node of the tree can be linked back}
\tcc*[r]{induction}

      {\bf if} {\code{is\_closed}(\utree{})} {\bf then } {\Return{{\unsat} };} %\hfill \text{check if the tree is closed} %%\tcc*{\unsat}}

	 \Else{
       %$(\D{:}l_i) {\leftarrow} \code{choose\_bfs}(\utree{});  $ \hfill \text{select a leaf and a predicate to unfold} %%\tcc*[r]{choose an open leaf}

	  % $ i {\leftarrow} i{+}1 $ \;
       $ \utree{}  {\leftarrow} \code{\unfoldsl}(\utree{}) $\tcc*{expand}
% \hfill \text{select a leaf and grow it with new leaves}
      }
%   }
%  {\Return{{\unsat} }};
 }
 \caption{Decision Algorithm ~{\algonameesl}}\label{algo.s2.sat} 
\end{algorithm}


==> sat-prm.tex <==
%% An overview of
The decision procedure in {\toolname} named {\algonameesl}
 is presented in Algorithm~\ref{algo.s2.sat}.
It takes a query $\D$, which is a formula in our assertion language, as well as a place holder $[]$ for a counterexample as inputs. It has two possible outcomes: % (if it terminates):
 {\sat} with a counterexample \form{\xi} (i.e., a sequence of statements
starting from the entry point to the error statement)
 or {\unsat} with a cyclic proof. %, a proof of induction.
 If it does not terminate after some threshold time units, we conclude the result is \code{UNKNOWN}.

At line 1, an execution tree with only one root node $\D$ is constructed. The loop (lines 2-11) then iteratively grows the tree while attempting
to establish a {\sat} proof or a {\unsat} proof.
In particular, at line 3, it checks whether
there is an error or not using a function \code{\uosl}(\utree{}).
 Function {\uosl} focuses on those leaf nodes which do not contain inductive predicates (referred to as base formulas).
%or do contain an error (referred to as error formulas).
If one of the leaf nodes is proved to be satisfiable, the algorithm returns {\sat} (line 4) together with the satisfiable node
%(obtained by using function {\algonamesl})
 as a counterexample (obtained by using function \code{get\_error}). Otherwise, those leaf nodes
are marked as closed.
 At line 5, function {\oosl} prunes infeasible execution traces.
Afterwards, every remaining leaf node is checked to see if it can be linked-back (to another node in the tree) to establish
a cyclic proof through function {\lbsl}.
At line 7, it checks whether the tree is closed (i.e. all leaf nodes are either marked closed or can be linked-back) and returns {\unsat} if so.
Otherwise, at line 9, it chooses a leaf which is neither marked closed nor linked-back and grows the tree by unfolding the inductive predicate in the node using function \code{\unfoldsl}. Afterwards, the same process is repeated until either {\sat} or {\unsat} is returned or a timeout occurs.
Details of function \code{\uosl} and \code{\lbsl} are discussed in Section
\ref{sat.base} and~\ref{sat.ind} respectively. In the following we present details of
function \code{\oosl} and \code{\unfoldsl}.

\input{sat-algo}


==> slldll.tex <==
\hide{
/ list(x)
node prev = x;
while (x != null) {
        x = x-> next;
        x -> prev = prev;
        prev = x;   
}
}

\begin{figure}
%% \begin{wrapfigure}{l}{0.47\textwidth}
\begin{center}
%%\caption{Motivating Example.}\savespace
%%\begin{minipage}{0.99\textwidth}
%%\begin{frameit} 
\begin{small} \[
\begin{array}{l}
 \code{~~\structd~\{int ~ val;~ \structd ~{\sep} next;\}} \\
%
\begin{array}{ll}
1 & \code{\structd{\sep}~sll(int ~ i)\{} \\
2 & \code{~~ if(i{==}0)~ return~ \code{NULL};}  \\
3 & \code{~~ else~\{}\\
4 & \code{~~~~ \structd ~ {\sep}n{=}(\structd{\sep})}\\
5 & \code{\quad~~~  malloc(sizeof(\structd));} \\
6 & \code{~~~~ n{\der}val{=}i; ~ n{\der}next{=}sll(i{-}1);} \\
%%4 & return ~new ~node(i{,}sll(i{-}1));\}}\\
7 & \code{~~~~return~n;\}\}} \\
 & \\
%
8 & \code{int~main(int ~n)\{} \\
%% 2 & \code{~~ int ~n{=} int\_nondet();}  \\
9 & \code{~~ \structd~{\sep}x;}  \\
10 & \code{~~ if(n{\leq}0) ~return~0;}  \\
11 & \code{~~ x{=}sll(n);}  \\
12 & \code{~~while(x) \{}  \\
13 & \code{~~~~ \structd~{\sep}tmp{=}p;}  \\
14 & \code{~~~~if(x{\der}val{<}0) ~ ERROR();}  \\
15 & \code{~~~~x{=}x{\der}next;}  \\
15 & \code{~~~~free ~ tmp;}  \\
17 & \code{~~ \};}  \\
18 & \code{~~ return ~1;} \\
19  & \}
\end{array} \\
%%\text{}\\
\text{\qquad \qquad \qquad~~~~~ a) C program} \\
\text{}\\
%%%%%%%%%%%%%%%%%%%%%%%%%
%%\begin{array}{l}
\code{~~data~node\{int ~ val;~~node~ prev;~~node~ next;\}} \\
\begin{array}{ll}
1 & \code{node~sll(int ~ i)\{} \\
%%  & \code{~~node~\res};\\
  & \code{~~bool~b_1{=}i{==}0};\\
2 & \code{~~ if(b_1)~ \res{=}\nil;}  \\
3 & \code{~~ else~\{}\\
 & \code{~~~~ int~i_3;~node~n_2,~n;}\\
& \code{~~~~ i_3{=}i{-}1}\\
 & \code{~~~~ n_2{=}sll(i_3)}\\
4 & \code{~~~~n{=} ~new ~node(i{,}n_2);}\\
7 & \code{~~~~\res{=}n;\}\}} \\
%% & \code{~~return~\res;\}} \\
%%\end{array}
\end{array}\\
\text{}\\
\text{ ~~~~    b) core program of \code{node} and \code{sll2dll} procedure} \\
\text{}\\
%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{array}{l}
\defpred~\form{\seppred{sll}{i{,}\res{,}\error}} ~\equiv~
\form{\emp {\wedge}\res{=}\nil {\wedge} i{=}0 {\wedge}\error{=}0} \\ %% \form{~~~|~ \res{=}\nil {\wedge} i{=}0} \\
~~ {\vee} \form{~{\exists} ~i_1{,}r {\cdot}~ \sepnode{\res}{node}{i{,}\anon{,}r} {\sep}
\seppred{sll}{i_1{,}r{,}\error}_{\_}^0 {\wedge}i{\neq}0{\wedge} i_1{=}i{-}1} \\
%% \form{~ |~ \res{\neq}\nil {\wedge} i{>}0} \\
  ~~ \invo{:}~i{\geq}0 {\wedge} \error{=}0;
\\
\text{ }
\\
\defpred~\form{\seppred{inv_{12}}{x{,}x'{,}\error}} ~\equiv~
 \form{\emp {\wedge} x{=}\nil  {\wedge}x'{=}x {\wedge} \error{=}0} \\%% \form{  \qquad|~ p{=}\nil {\wedge} \res{=}1 } \\
~~ {\vee} ~ {\dangl{x}{\wedge} x{\neq}\nil  {\wedge} \error{=}1} \\ %% \form{\qquad|~ p{\neq}\nil {\wedge} \res{=}0} \\
~~ {\vee} r_1{,}p_2{\cdot}
 \form{{\neg}\dangl{x} {\sep}\seppred{inv_{12}}{x_1{,}x'{,}\error}_{\_}^0
  {\wedge}x{\neq}\nil {\wedge} x_1{=}x.next};
 %% \qquad \form{|~ p{\neq}\nil {\wedg
\\
\text{ }
\\
\defpred~\form{\seppred{main}{n{,}\res{,}\error}} ~\equiv~
\form{ \emp {\wedge}n{<}0 {\wedge} \res{=}0 {\wedge} \error{=}0} \\
~~ {\vee} ~\form{\exists \error_1{,}\error_2 {\cdot}\seppred{sll}{n{,}x{,}\error_1}_{\_}^0
{\sep} \seppred{inv_{12}}{x{,}x'{,}\error_2}_{\_}^1 {\wedge}n{\geq}0
{\wedge}\error_1{=}0 {\wedge}\error_2{=}1 {\wedge} \error{=}1 } \\
~~ {\vee} ~\form{\exists \error_1{,}\error_2 {\cdot}\seppred{sll}{n{,}x{,}\error_1}_{\_}^0
{\sep} \seppred{inv_{12}}{x{,}x'{,}\error_2}_{\_}^1 {\wedge}n{\geq}0
{\wedge}\error_1{=}0 {\wedge}\error_2{=}0 {\wedge} \error{=}0 } ;\\
\text{ }
\\
\form{\seppred{main}{n_0{,}\res_0{,}\error_0}^0_0 {\wedge}\error_0{=}1}.
\end{array}\\
\text{}\\
\text{\qquad \qquad~~~~~\qquad c) Verification Condition} \\
 \end{array}
%%\quad
%%%%%%%%%%%%%%%%%%%%%%%%%
%% \begin{array}{l}
%%  \code{~~data~node\{int ~ val;}\\
%%  \code{\qquad \quad node~ next;\}} \\
%% %
%% \begin{array}{ll}
%% 1 & \code{node~sll(int ~ i)\{} \\
%%   & \code{~~node~\res};\\
%%   & \code{~~bool~b_1{=}i{==}0};\\
%% 2 & \code{~~ if(b_1)~ \res{=}\nil;}  \\
%% 3 & \code{~~ else~\{}\\
%%  & \code{~~~~ node~n_2{=}sll(i{-}1)}\\
%% %% 5 & \code{\quad~~~  malloc(sizeof(\structd));} \\
%% %% 6 & \code{~~~~ n{\der}val{=}i; ~ n{\der}next{=}sll(i{-}1);} \\
%% 4 & \code{~~~~node~n{=} ~new ~node(i{,}n_2);}\\
%% 7 & \code{~~~~\res{=}n;\}} \\
%%  & \code{~~return~\res;\}} \\
%%  & \\
%% %
%% 8 & \code{int~main(int ~n)\{} \\
%% %% 2 & \code{~~ int ~n{=} int\_nondet();}  \\
%%   & \code{~~int~\res};\\
%%   & \code{~~bool~b_3{=}n{<}0};\\
%% 9 & \code{~~ if(b_3) ~\res{=}0;else\{\}}  \\
%% 10 & \code{~~ node~x{=}sll(n);}  \\
%% 11 & \code{~~ node~p{=}x, tmp{=}x;}  \\
%% 12 & \code{~~while(tmp) \{;}  \\
%% 13 & \code{~~~~tmp{=}tmp{.}next;}  \\
%% 14 & \code{~~~~tmp{.}prev{=}p;}  \\
%% 15 & \code{~~~~p{=}tmp;}  \\
%% 16 & \code{~~ \};}  \\
%% 17 & \code{~~while(p{!=}x) \{}  \\
%% 18 & \code{~~~~if(p{.}val{<}0) ~ ERROR();}  \\
%% 19 & \code{~~~~free ~ p;}  \\
%% 20 & \code{~~~~p{=}p{.}prev;}  \\
%% 21 & \code{~~ \};}  \\
%% 22 & \code{~~ free~x;}  \\
%% 23 & \code{~~ return ~1;} \\
%% 24  & \}
%% \end{array}
%%  \end{array}
%% \\
%%%%%%%%%%%%
%% \quad
%% \begin{array}{l}
%% \defpred~\form{\seppred{sll}{i{,}\res}} ~\equiv~
%% \form{\emp {\wedge}\res{=}\nil {\wedge} i{=}0} \\ %% \form{~~~|~ \res{=}\nil {\wedge} i{=}0} \\
%% ~~ {\vee} \form{~{\exists} ~i_1{,}r {\cdot}~ \sepnode{\res}{node}{i{,}r} \sep
%% \seppred{sll}{i_1{,}r}_{\_}^0 {\wedge}i{\neq}0{\wedge} i_1{=}i{-}1} \qquad
%% %% \form{~ |~ \res{\neq}\nil {\wedge} i{>}0} \\
%%   ~~ \invo{:}~i{\geq}0;
%% \\
%% \defpred~\form{\seppred{test_v}{p{,}\res}} ~\equiv~
%% \form{ p{=}\nil {\wedge} \res{=}1} %% \form{  \qquad|~ p{=}\nil {\wedge} \res{=}1 } \\
%% ~~ {\vee} ~ { p{\neq}\nil {\wedge} p.val{<}0 {\wedge}
%%  \res{=}0} \\ %% \form{\qquad|~ p{\neq}\nil {\wedge} \res{=}0} \\
%% ~~ {\vee} \code{
%%     p{\neq}\nil {\wedge} p.val{\geq}0
%%  {\wedge}\seppred{test_v}{p.next{,}\res}_{\_}^0} \qquad
%%  %% \qquad \form{|~ p{\neq}\nil {\wedge} 0{\leq}\res{\leq}1} \\
%%  ~~ \invo{:}~0{\leq}\res{\leq}1; \\
%% \end{array}
\] %%\savespace
\end{small}
%%\end{frameit}
%%\end{minipage}%  \savespace \savespace  %% \saveone
\savespace \savespace
\caption{sll2dll Example.}
\label{fig.mov.slldll}
\end{center} % \saveone %%\savespace \savespace
\end{figure}


==> symex-loop.tex <==
\savespace\[\savespace
\hlr{WHILE}{
\begin{array}{c}
i)~~  V_1{=}\{x_1{,}..{,}x_m\} \quad
V_2{=}\{v_1{,}..{,}v_n{,}\error\} \quad
 \D_0{=}\emp{\wedge}{\neg} v'{\wedge}\nochange(V_2){\wedge}\error'{=}0{:}[2] \\
 \htriple{\emp{\wedge}\nochange(V_2){\wedge}v'{:}[1]}{e}{\bigvee \D_i{:}l_i} \quad  \D_i^e{=}\code{set}(\D_i) \\
\myit{W}{=}\primeV(V_1) \quad \defpred~ \seppred{{inv_p}}{v_1{,}..{,}v_n{,}x_1{,}..{,}x_m{,}v'_1{,}..{,}v'_n{,}\error}
 {\equiv} {(\D_0{:}[2]  {\vee} \bigvee ~{\exists}  \myit{W}{\cdot}\D_i^e{:}l_i)} \\
ii)~  \fresh ~ e ~~ \fresh~ w_1{,}..{,}w_n \quad i {\in} 0,1 \quad \form{l} \text{ is an increasing number}
 \quad \rho{=}w_1/v_1,..,w_n/v_n \\
 \pure{=}e{=}i {\wedge}\error'{=}i \quad
 \quad \D_{1_i}{=}\exists e{\cdot}\D[\rho] {\sep}
  (\seppred{{inv_p}}{w_1{,}..{,}w_n{,}x'_1{,}..{,}x'_m{,}v'_1{,}..{,}v'_n{,}e}_{\_}^l{\wedge}\pure) \\
\end{array}}
{\htriple{\D{:}l}{\mywhile{v}{e}}{(\D_{1_0}{:}l) ~{\vee}~ (\D_{1_1}{:}l)}}
\]
\code{while} loops are encoded through two steps as follows.
(i) First, encoding of loop body is similar
 to the encoding of a recursive function.
Each loop is transformed into an inductive predicate.
Arguments of this predicate are those which are either read \form {V_1} or
written in the loop body \code{e}, or primed version
of the written arguments. While \form{\D_0} is the encoding for the loop exit,
\form{\bigvee ~{\exists}  \myit{W}{\cdot}\D_i^e}
 is the encoding for the loop body.
(ii) Second, the loop invariant is combined into current states like the encoding of
the function call.


==> symex.triple.tex <==
\begin{figure*}[thb]
\begin{center}
%% \savespace
%% \begin{minipage}{1\textwidth}
%% \begin{frameit}\vspace*{-2.5mm}\savespace
%% \saveone\[\saveone
%% \hlr{LOCAL}
%% {t{\not\in} Node ~~ \htriple{\D{:}l}{e}{\D_1{:}l_1} }
%%  {\htriple{\D{:}l}{\{t~v;~e\}}{\exists\,v,v'{\cdot}\D_1{:}l_1}}
%% \quad
%% \hlr{LOCAL-PTR}
%% {t{\in} Node ~~ \htriple{\D{\sep}\dangl{v}{:}l}{e}{\D_1{:}l_1} }
%%  {\htriple{\D{:}l}{\{t~v;~e\}}{\exists\,v,v'{\cdot}\D_1{:}l_1}}
%% \]
\[
\hlr{ASSUME}{\sigma{=} \circ \{v'/v ~|~ v\in \FV(\pure) \}}{\htriple{\D{:}l}{\code{assume}~\pure}{(\D{\wedge}(\pure \sigma)){:}l}}
%% \qquad
%% \hlr{ASSERT}{\sigma{=} \circ \{v'/v ~|~ v\in \FV(\pure) \}}{\htriple{\D{:}l}{\code{assert}~\pure}{(\D{\wedge}{\neg}(\pure\sigma){\wedge}\error'{=}1){:}l ~\vee~ \D{:}l} }
\]
\[
\hlr{IF}{
\begin{array}{c}
\htriple{\D{\wedge}v'{:}(l{::}1)}{e_1}{\D_1{:}l_1} \quad%\\
\htriple{\D{\wedge}{\neg}v'{:}(l{::}2)}{e_2}{\D_2{:}l_2}
\end{array}}
{\htriple{\D{:}l}{\myif{v}{e_1}{e_2}}{\D_1{:}l_1{\vee}\D_2{:}l_2}}
\qquad
\hlr{VAR}{\D_1{=}(\D{\wedge}\res{=}v')}{\htriple{\D{:}l}{v}{\D_1{:}l}}
\]
\[
\hlr{SEQ}{\htriple{\D{:}l}{e_1}{\D_1{:}l_1} \quad \htriple{\D_1{:}l_1}{e_2}{\D_2{:}l_2}}
{\htriple{\D{:}l}{e_1;e_2}{\D_2{:}l_2}}
\qquad
\hlr{NEW}{
\D_1{=}(\D\,{\sep}\,\sepnodeF{\res}{c}{v'_1{,}..{,}v'_n})}
{\htriple{\D{:}l}{\new~c(v_1,..,v_n)}{\D_1}{:}l}
\]
\[
\hlr{ASSIGN}{\htriple{\D{:}l}{e}{\D_1{:}l_1} ~~ \D_2{=}
\exists \res{,}
r{\cdot}(\D_1[r/v'] {\wedge}
v'{=}\res)  ~~\fresh~r} {\htriple{\D{:}l}{v{:=}e}{\D_2{:}l_1}}
\qquad \hlr{CONST}{\D_1{=}(\D {\wedge} \eq{\tau}{\res}{k})} {\htriple{\D{:}l}{k^\tau}{\D_1{:}l}}
\]
\[
\hlr{CALL}{
 %%t~mn((t_i~v_i)^n_{i{=}1})~\{..\}{\in} \sc{PG} \quad
 \D_{1_i}{=}\exists e{\cdot}\D {\sep}  \seppred{ \myit{mn}}{v_1'{,}..{,}v'_n{,}\res{,}e}_{\_}^n{\wedge}e{=}i {\wedge}\error'{=}i {:}l \\
 \fresh ~ e \quad i {\in} \{0{,}1\} \quad \form{n} \text{ is an increasing number}}
{\htriple{\D{:}l}{mn(v_1..v_n)}{\D_{1_0} ~{\vee}~ \D_{1_1}}}
\qquad
\hlr{LOCAL-PTR}
{t{\in} Node ~~ \htriple{\D{\sep}\dangl{v'}{:}l}{e}{\D_1{:}l_1} }
 {\htriple{\D{:}l}{\{t~v;~e\}}{\exists\,v,v'{\cdot}\D_1{:}l_1}}
\]
\[
\hlr{LOOP}{
\begin{array}{c}
i)~~  V_1{=}\{x_1{,}..{,}x_m\} ~~
V_2{=}\{v_1{,}..{,}v_n{,}\error\} ~~\pure_{e}{=} \nochange(V_2)\quad
  \htriple{\emp{\wedge}\pure_e{\wedge}v'{:}[1]}{e}{\bigvee \D_i{:}l_i} \quad
 \D_i^e{=}\code{encodeL}(\D_i) \\
\myit{W}{=}\primeV(V_1) \quad
\D_0{=}\emp{\wedge}{\neg} v'{\wedge}\pure_e{\wedge}\error'{=}0{:} \quad
 \defpred~ \seppred{{inv_p}}{v_1{,}..{,}v_n{,}x_1{,}..{,}x_m{,}v'_1{,}..{,}v'_n{,}\error}
 {\equiv} {(\D_0{:}[2]  {\vee} \bigvee ~{\exists}  \myit{W}{\cdot}\D_i^e{:}l_i)} \\
ii)~  \fresh ~ e ~~ \fresh~ w_1{,}..{,}w_n \qquad i {\in}\{0{,}1\} \quad \form{n} \text{ is an increasing number across program}
 \qquad \sigma{=}[w_1/v_1,..,w_n/v_n] \\
 \pure_i{=}e{=}i {\wedge}\error'{=}i \quad
 \qquad \D_{1_i}{=}\exists e{\cdot}\D\sigma {\sep}
  (\seppred{{inv_p}}{w_1{,}..{,}w_n{,}x'_1{,}..{,}x'_m{,}v'_1{,}..{,}v'_n{,}e}_{\_}^n{\wedge}\pure_i) \\
\end{array}}
{\htriple{\D{:}l}{\mywhile{v}{e}}{(\D_{1_0}{:}l) ~{\vee}~ (\D_{1_1}{:}l)}}
\]
\[
\hlr{FREE}{
\D_1{=}(\D{\wedge} x'{=}\nil{\wedge}e'{=}1) \quad \D_2{=}\D{\wedge}{\dangl{x'}}{\wedge}{e'{=}1}
\quad \D_3{=}\D[w/x']{\wedge}{\neg\dangl{w}}{\wedge}{\dangl{x'}}{\wedge}w{\neq}\nil \quad
~where ~w~is~\fresh
}
{\htriple{\D{:}l}{\code{free}~x}{\D_1}{:}l ~{\vee}~ \D_2{:}l ~{\vee}~\D_3{:}l}
\]
\[
\hlr{LOAD}{
\pure_1{=}{v'{=}\nil}{\wedge}{e'{=}1} ~~
\pure_2{=}{\dangl{v'}}{\wedge}{e'{=}1} \\
\quad \pure_3 {=} {\neg\dangl{v'}}{\wedge}v'{\neq}\nil{\wedge}
\sepnodeR{v'}{f_i}{\res}{k} %%  \res{=}v'.f_i
}
{\htriple{\D{:}l}{v{\der}f_i}{(\pure_1}{\vee}\pure_2{\vee}\pure_3){\wedge}\D{:}l}
\qquad
\hlr{STORE}{
\pure_1{=}{v'{=}\nil}{\wedge}{e'{=}1} ~~
\pure_2{=}{\dangl{v'}}{\wedge}{e'{=}1}  \\
 \quad \pure_3 {=} {\neg\dangl{v'}}{\wedge}v'{\neq}\nil{\wedge}
\sepnodeW{v'}{f_i}{v'_0}{k} %% v'.f_i{=} v'_0
}
{\htriple{\D{:}l}{v{\der}f_i{:=}v_0}{(\pure_1}{\vee}\pure_2{\vee}\pure_3){\wedge}\D{:}l}
\]
%% \[
%% \begin{array}{l}
%%\text{Local Variable Declaration: } \\ \quad
%%  {\htriple{\D{:}l}{\{t~v;e\}}{\exists\,v,v'{\cdot} \D_1{:}l}}, ~\text{where} %%\\
%%  {t{\not\in} Node, \htriple{\D}{e}{\D_1}}
%% \text{  or  }
%% {t{\in} Node, \htriple{\D{\sep}\dangl{v}}{e}{\D_1} } \\
%% %% \\
%% %% \text{ }\\
%% %% \text{Variable and Constant:}\\
%% %% \quad
%% {\htriple{\D{:}l}{v}{(\D{\wedge}\res{=}v'){:}l}} 
%% \qquad \quad
%% {\htriple{\D{:}l}{k^\tau}{(\D {\wedge} \eq{\tau}{\res}{k}){:}l}}
%% \\
%% %%\text{ }\\
%% %% \text{Assumption: }
%% {\htriple{\D{:}l}{\code{assume}~\pure}{(\D{\wedge}\pure){:}l}}
%% %% \text{ }\\
%% \qquad \quad
%% %% \text{Assertion: }
%% {\htriple{\D{:}l}{\code{assert}~\pure}{(\D{\wedge}\neg\pure{\wedge}\error'{=}1){:}l}}
%%\text{ }\\
%%\\
%%\text{If: }
%%  \htriple{\D{:}l}{\myif{v}{e_1}{e_2}}{(\D_1{:}l_1){\vee}(\D_2{:}l_2)}, \text{ where} \\
%% \quad \htriple{(\D{\wedge}v'){:}(l::1)}{e_1}{\D_1{:}l_1} \text{ and } 
%% \qquad \htriple{(\D{\wedge}{\neg}v'){:}(l::2)}{e_2}{\D_2{:}l_2}
%%\\
%%\text{ }\\
%%\text{Sequence: }
%%  {\htriple{\D{:}l}{e_1;e_2}{\D_2:l_2}}, ~\text{where } %% \\
%% \quad{\htriple{\D{:}l}{e_1}{\D_1{:}l_1} \text{ and } \htriple{\D_1{:}l_2}{e_2}{\D_2{:}l_2}}
%% \\
%% \text{ }\\
%% \text{Function Call: } 
%% {\htriple{\D{:}l}{mn(v_1..v_n)}{\D_{1_0} ~{\vee}~ \D_{1_1}}}, \text{ where} \\
%% \quad \D_{1_i}{=}\exists e{\cdot}\D {\sep}  \seppred{ \myit{mn}}{v_1'{,}..{,}v'_n{,}\res{,}e}_{\_}^l{\wedge}e{=}i {\wedge}\error'{=}i{:}l %%\\
%% \quad \fresh ~ e \quad i {\in} 0,1 \quad \form{l} \text{ is an increasing number}
%% \\
%%\text{ }\\
%%\text{Assignment: } 
%%  {\htriple{\D{:}l}{v{:=}e}{\D_2{:}l_1}}, \text{ where} %%\\
%% \quad {\htriple{\D{:}l}{e}{\D_1{:}l_1} \qquad \D_2{=}
%% \exists \res{,}r{\cdot}([r/v']\D_1 {\wedge} v'{=}\res)  ~\fresh~r}
%% \\
%%\text{ }\\
%%\text{Heap Allocated: }\\ \quad
%%  {\htriple{\D{:}l}{\new~c(v_1,..,v_n)}{\D{\sep}\sepnodeF{\res}{c}{v'_1{,}..{,}v'_n}{:}l}}
%% \\
%%\text{ }\\
%% \text{Heap Deallocated: }
%%  {\htriple{\D{:}l}{\code{free}~x}
%% {(\D_1{:}l) {\vee} (\D_2{:}l) {\vee} (\D_3{:}l)}}, \quad
%%  \text{ where} ~~ \D_1{=}\D{\wedge}{x'{=}\nil}{\wedge}{e'{=}1} \quad
%% \D_2{=}\D{\wedge}{\dangl{x'}}{\wedge}{e'{=}1}\\
%%  \quad\D_3{=}\D[w/x']{\wedge}{\neg\dangl{w}}{\wedge}{\dangl{x'}}{\wedge}w{\neq}\nil
%% \text{ where } \fresh ~w
%% \\
%%\text{ }\\
%% \text{Field Load: }
%%  {\htriple{\D{:}l}{v{\der}f_i}{(\D_1{:}l) {\vee}
%%  (\D_2{:}l) {\vee} (\D_3{:}l)}},
%%  \text{ where}~~
%%  \D_1{=}\D{\wedge}{v'{=}\nil}{\wedge}{e'{=}1} \quad
%% \D_2{=}\D{\wedge}{\dangl{v'}}{\wedge}{e'{=}1} \\
%% \quad \D_3 {=} \D{\wedge}{\neg\dangl{v'}}{\wedge}v'{\neq}\nil{\wedge}\res{=}v'.f_i
%% %\]
%% \\
%%\text{ }\\
%% \text{Field Store: }
%%  {\htriple{\D{:}l}{v{\der}f_i{:=}v_0}
%% {(\D_1{:}l) {\vee} (\D_2{:}l) {\vee} (\D_3{:}l)}},
%%  \text{ where} ~~ \D_1{=}\D{\wedge}{v'{=}\nil}{\wedge}{e'{=}1} ~~
%% \D_2{=}\D{\wedge}{\dangl{v'}}{\wedge}{e'{=}1}  \\
%%  \quad \D_3 {=} \D{\wedge}{\neg\dangl{v'}}{\wedge}v'{\neq}\nil{\wedge} v'_0{=}v'.f_i
%% \\
%% \text{Loop: } {\htriple{\D}{\mywhile{v}{e}}{ \constr}} \text{ where }
%% V_1{=}\{v_1{,}..{,}v_n{,}\error\} ~~ \myit{W}{=}\primeV(V_1)\\
%%  ~~~V_2{=}\{x_1{,}..{,}x_m\}
%%   \quad \D_0{=}\emp{\wedge}{\neg} v'{\wedge}\nochange(V_1){\wedge}\error'{=}0 \\
%% \htriple{\emp{\wedge}\nochange(V_2){\wedge}v'}{e}{\bigvee \D_i} \quad  \D_i^e{=}\code{set}(\D_i) \\
%%  \defpred~ \seppred{{inv_p}}{v_1{,}..{,}v_n{,}x_1{,}..{,}x_m{,}v'_1{,}..{,}v'_n{,}\error}
%%  {\equiv} {(\D_0  {\vee} \bigvee ~{\exists}  \myit{W}{\cdot}\D_i^e)\,} \\
%% \htriple{\D}{e}{{\bigvee}\D_i}  ~~
%% \end{array}
%% \]
%% \[
%% %{{\bf meth~decl~rule}}
%% \hlr{METH}{ V{=}\{v_1{,}..{,}v_n{,}\error{,}\res\} ~~  \myit{W}{=}\primeV(V) ~~ \D{=}\emp{\wedge}\nochange(V) ~~
%% \htriple{\D}{e}{\bigvee \D_i} \\ \defpred~ \seppred{ \myit{mn\_v}}{v_1{,}..{,}v_n,\error{,}\res} ~{\equiv}~ {(\bigvee ~{\exists} \myit{W}{\cdot}\D_i)\,}}{\vdash
%% t_0~\myit{mn}(t_1~v_1,..,t_n~v_n)~\{e\}}
%% \]
%% \end{frameit}%%\vspace*{-3mm}
%% \end{minipage}
\caption{Encoding VC via Symbolic Execution}\label{fig.ntyperules}
\end{center}
\end{figure*}


==> tll.tex <==
An example is the method below
to manipulate
a tree
whose leaf nodes are linked as a list.
\begin{small}
\[
\begin{array}{l}
\code{\structt~\{int ~val{,}~ \, \structt\pntr~parent; \structt \pntr~l;~\structt \pntr~r; ~\structt\pntr~next\}}\\
\begin{array}{ll}
\begin{array}{ll}
8 & \code{int~main(int ~n)\{} \\
9 & \code{~~ \structt~{\sep}x{,}~{\sep}lm;}  \\
10 & \code{~~ if(n{\leq}0) ~return~0;}  \\
11 & \code{~~ x{=}bin\_tree(n);}  \\
12 & \code{~~  lm{=}tll(x{,}NULL{,}NULL)} \\
14 & \code{~~if(lm{\der}val{<}0) ~ ERROR();}  \\
17 & \code{~~ return ~1;\}} \\
\end{array} &
\begin{array}{l}
\code{\structt\pntr~tll(\structt\pntr~x,\structt\pntr~p,\structt\pntr~t)\{}\\
\code{~~x{\der}parent=p;}\\
\code{~~if~(x{\der}r{==}NULL)~\{%}\\
  ~x{\der}next {=} t;return~x;\}}\\
\code{~~else~\{}%\\
\code{~~\structt\pntr~lm=tll(x{\der}r,x,t);}\\
\code{~~~~return~tll(x{\der}l,x,lm);\}}\\
\code{\}}
\end{array}
\end{array}
\end{array}
\]
\end{small}
%
Our approach to modular shape analysis would
introduce an unknown pre-predicate
\code{H} (as the pre-condition), and an unknown post-predicate \code{G} (as the post-condition),
 as shown below,
where \code{\res} is the method's result.
%
\begin{small}
\[ \savespace
\requires \quad \seppred{H}{x,p,t} \qquad\quad
\ensures \quad\seppred{G}{x,p,\res,t}
\vspace{-1mm}
\]
\end{small}
%
\indent Using Hoare-style verification and a new
second-order bi-abduction entailment procedure, we would derive
a set of relational assumptions for the two unknown predicates.
These derived assumptions are to ensure memory safety, and
can be systematically transformed into concise predicate
definitions for the unknown predicates, such as:
%
 \begin{small}\savespace
 \[
 \begin{array}{l}
\seppred{H}{x{,}p{,}t} \equiv   
\sepnode{x}{tree}{\DP_p{,}\DP_l{,}r{,}\DP_n} \wedge    \code{r}{=}\nil\\
\qquad\qquad \vee~
\sepnode{x}{tree}{\DP_p{,}l{,}r{,}\DP_n} {\sep}  
\seppred{H}{l{,}x{,}lm} {\sep} \seppred{H}{r{,}x{,}t}\wedge
\code{r}\ne \nil 
\\[3pt]
\seppred{G}{x{,}p{,}\res{,}t} \equiv \sepnode{x}{tree}{p{,}\DP_l{,}r{,}t}
\wedge \res{=}\code{x} {\wedge} \code{r}{=}\nil\\
\qquad\qquad\vee~ \sepnode{x}{tree}{p{,}l{,}r{,}\DP_n}
 {\sep}  \seppred{G}{l{,}x{,}\res{,}lm} {\sep} \seppred{G}{r{,}x{,}lm{,}t} {\wedge} 
\code{r}{\ne}\nil 
 \end{array}
 \]  \savespace
 \end{small}

\begin{wrapfigure}{l}{0.4\textwidth}
\savespace\savespace
 \vspace*{-6mm}
\savespace \savespace
\begin{center}
    \includegraphics[width=48mm]{tll}
\savespace \savespace \savespace \savespace
\caption{An example of \code{\seppred{G}{x{,}p{,}\res{,}t}}}
\label{fig:sec1:tll}
\end{center}
\vspace{-8mm}
\savespace 
%% \savespace
\end{wrapfigure}
The derived pre-predicate \code{H} captures a binary tree-like shape that
would be traversed by the method.  \code{\sepnode{x}{tree}{\DP_p{,}\DP_l{,}r{,}\DP_n}}
denotes that \code{x} refers to a \code{tree} node with its \code{parent},\code{l},\code{r} and \code{next} fields
being \code{\DP_p}, \code{\DP_l}, \code{r} and \code{\DP_n}, respectively.
We use dangling references,
such as \code{\DP_l,\DP_p,\DP_n}, as generic markers that denote 
field pointers that are not traversed by the method. 
Thus no assertion can be made on any of the \code{\DP} pointers.  
The post-predicate \code{G}, illustrated in Fig~\ref{fig:sec1:tll}, 
adds \code{parent} field links for all nodes,
and \code{next} field links for just the leaves.
\footnote{Note that new links formed by the method are colored in red.
}

\noindent Current shape analysis mechanisms \cite{predator,Berdine:CAV11,CalcagnoDOY09}
are unable to infer pre/post specifications 
that ensure
memory-safety for such complex examples.


==> witness.tex <==
%% \begin{algorithm}[ht]
%%   \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
%%   \SetAlgoLined

%%  \Input{($\xi$, \code{loc}, $\sc{Prog}$)} \Output{\code{res}}
%%    $(\code{proc\_name}, l) {\leftarrow} \code{hd}(\xi)$;
%%    $\xi {\leftarrow} \code{tail}(\xi) $ %%\tcc*{initialize}

%%    $ \code{res} {\leftarrow} \emptyset; $; $ W  {\leftarrow} \emptyset $

%%  \While {$\xi {\not=} \emptyset ~{\wedge}~ l{\not=} \emptyset ~{\wedge}~ W{\not=} \emptyset $}
%%  {
%%   $ \code{e} {\leftarrow} next(\code{proc\_name})$;

%%   $ \code{res} {\leftarrow} push(\code{res}{,} \code{e}) $

%%    \While{\code{e} ${\not=}$ \code{return}}
%%    {
%%      \Switch{\code{e}}{
%%        \Case{\code{if~ b~then ~e_1~else~e_2}}{

%%        }
%%        \Case{\code{mn(...)}}{
%%        }
%%        \Other{
%%        }
%%      }
%%    }

%%     (\code{is\_sat},\utree{i}) {$\leftarrow$} \code{\uot}(\utree{i});  %%\tcc*[r]{check {\sat}}

%%    {\bf if} {\code{is\_sat}} {\bf then }
%%    {\Return{${\sat}$} \tcc*{\sat}}
%%    \Else{
%%      $\utree{i} {\leftarrow} \code{\oot}(\utree{i});  $ %%\tcc*[r]{prune {\unsat}}

%%       $ \utree{i}  {\leftarrow} \code{link\_back}(\utree{i}) $ \tcc*[r]{cyclic proof}
%%       {\bf if} {\code{is\_closed}(\utree{i})} {\bf then } {\Return{{\unsat} }\tcc*{\unsat}}
%%    }
%%  }
%%  \caption{Error Witness Generation}\label{algo.witness}
%% \end{algorithm}

%%CPAChekcer \cite{Dirk:CAV:2015}, UAutomizer \cite{Heizmann:CAV:13}.

%% The procedure to generate problematic program path is desribed in Algorithm
%% \ref{algo.witness}.




